Dependency-Aware Software Requirements Selection using Fuzzy Graphs and Integer Programming

Software requirements selection aims to find an optimal subset of the requirements with the highest value while respecting the project constraints. But the value of a requirement may depend on the presence or absence of other requirements in the optimal subset. Such Value Dependencies, however, are imprecise and hard to capture. In this paper, we propose a method based on integer programming and fuzzy graphs to account for value dependencies and their imprecision in software requirements selection. The proposed method, referred to as Dependency-Aware Software Requirements Selection (DARS), is comprised of three components: (i) an automated technique for the identification of value dependencies from user preferences, (ii) a modeling technique based on fuzzy graphs that allows for capturing the imprecision of value dependencies, and (iii) an Integer Linear Programming (ILP) model that takes into account user preferences and value dependencies identified from those preferences to reduce the risk of value loss in software projects. Our work is verified by studying a real-world software project. The results show that our proposed method reduces the value loss in software projects and is scalable to large requirement sets.

==> lr1.tex <==
\begin{tabular}{|r|r|rrr|r|r|r|r|}
\hline
\textbf{Employed Model} &
  \textbf{Works} &
  \textbf{P1} &
  \textbf{P2} &
  \textbf{P3} &
  \textbf{P4} &
  \textbf{P5} &
  \textbf{P6} &
  \textbf{P7}
  \bigstrut\\
\hline
BKP &
   &
   &
   &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  
  \bigstrut\\
\hline
\multirow{5}[10]{*}{BKP-PC} &
   &
   &
   &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  
  \bigstrut\\
\cline{2-9} &
   &
   &
   &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  
  \bigstrut\\
\cline{2-9} &
   &
   &
   &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  
  \bigstrut\\
\cline{2-9} &
   &
   &
   &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  
  \bigstrut\\
\cline{2-9} &
   &
   &
   &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  
  \bigstrut\\
\hline
Increase/Decrease_Value_Of (subsets of size 2) &
   &
   &
   &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  
  \bigstrut\\
\hline
Increase/Decrease_Value_Of (subsets of any size) &
   &
   &
   &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  
  \bigstrut\\
\hline
\end{tabular}%


==> rq/rq_dars_ilp_sim.tex <==
\begin{itemize}[leftmargin=1.8cm]
	\itemsep0em 
	\hypertarget{RQ7}{ }
	\item[(\textbf{RQ7})] How is the performance of DARS-ILP affected by changing value dependencies, precedence dependencies and project constraints?  
	\hypertarget{RQ7.1}{ }
	\item[(\textbf{RQ7.1})] What is the impact of the value dependencies on the performance of DARS-ILP in the presence of various budget constraints?  
	\hypertarget{RQ7.2}{ }
	\item[(\textbf{RQ7.2})] What is the impact of the negative value dependencies on the performance of DARS-ILP in the presence of various budget constraints?  
	\hypertarget{RQ7.3}{ }
	\item[(\textbf{RQ7.3})] What is the impact of the precedence dependencies on the performance of DARS-ILP in the presence of various budget constraints? 
	\hypertarget{RQ7.4}{ }
	\item[(\textbf{RQ7.4})] What is the impact of the negative precedence dependencies on the performance of DARS-ILP in the presence of various budget constraints?
	\hypertarget{RQ7.5}{ }
	\item[(\textbf{RQ7.5})] What is the impact of the negative value dependencies in highly, moderately, or loosely interdependent value dependency graphs?
	\hypertarget{RQ7.6}{ }
	\item[(\textbf{RQ7.6})] What is the impact of the negative precedence dependencies in highly or loosely interdependent precedence dependency graphs?
\end{itemize}

==> rq/rq_dars_ip.tex <==
\begin{itemize}[leftmargin=1.8cm]
	\itemsep0em 
	\hypertarget{RQ1}{ }
	\item[(\textbf{RQ1})] What is the impact of using DARS-IP on the overall value of software products? 
	\hypertarget{RQ2}{ } 
	\item[(\textbf{RQ2})] What is the relationship between maximizing the accumulated value and overall value of software products?
	\hypertarget{RQ3}{ }
	\item[(\textbf{RQ3})] How effective is DARS-IP in mitigating the selection deficiency problem?
	\hypertarget{RQ4}{ }
	\item[(\textbf{RQ4})] What is the impact of value dependencies on the performance of DARS-IP? 
	\hypertarget{RQ5}{ }
	\item[(\textbf{RQ5})] How practical is DARS-IP for software projects?     
\end{itemize}

==> rq/rq_dars_mip.tex <==
\begin{itemize}[leftmargin=1.8cm]
	\hypertarget{RQ10}{ }
	\item[(\textbf{RQ10})] How effective is the DARS-MLP method in reducing the value loss?
\end{itemize}

==> table_cost_value.tex <==
\scriptsize\resizebox {0.6\textwidth }{!}{
\begin{tabular}{lllllll}
	\toprule[1.5pt]
	\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \textbf{$r_i$}} & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \textbf{$c_i$}} & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \textbf{$v_i$}} & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \textbf{$r_i$}} & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \textbf{$c_i$}} & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \textbf{$v_i$}} \\ \midrule
	$r_1$ & 05.00 & 10.00 & $r_{15}$ & 15.00 & 08.00 \\
	$r_2$ & 20.00 & 20.00 & $r_{16}$ & 13.00 & 10.00 \\
	$r_3$ & 00.00 & 04.00 & $r_{17}$ & 14.00 & 06.00  \\
	$r_4$ & 10.00 & 17.00 & $r_{18}$ & 03.00 & 10.00  \\
	$r_5$ & 01.00 & 03.00 & $r_{19}$ & 10.00 & 20.00  \\
	$r_6$ & 20.00 & 20.00 & $r_{20}$ & 07.00 & 20.00  \\
	$r_7$ & 06.00 & 15.00 & $r_{21}$ & 12.00 & 15.00  \\
	$r_8$ & 05.00 & 09.00 & $r_{22}$& 15.00 & 20.00  \\
	$r_9$ & 16.00 & 20.00 & $r_{23}$ & 08.00  & 20.00  \\
	$r_{10}$ & 10.00 & 16.00 & $r_{24}$ & 02.00  & 05.00 \\
	$r_{11}$ & 04.00 & 20.00 & $r_{25}$ & 10.00   & 00.00 \\
	$r_{12}$ & 03.00 & 10.00 &$r_{26}$ & 00.00 & 00.00  \\
	$r_{13}$ & 05.00 & 06.00 &$r_{27}$ & 01.00 & 00.00 \\
	$r_{14}$ & 07.00 & 08.00 &        &  &  \\[2pt] \midrule
	{\color[HTML]{000000} \textbf{Sum}} & {\color[HTML]{000000} 112.00} & {\color[HTML]{000000} 178.00} & {\color[HTML]{000000} -} & {\color[HTML]{000000} 110.00} & {\color[HTML]{000000} 134.00} \\ \bottomrule[1.5pt]
\end{tabular}

}

==> table_cs_dependencies.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
%\Huge
%\huge
%\LARGE
%\Large
%\large
%\normalsize (default)
%\small
%\footnotesize
%\scriptsize
%\tiny
\normalsize\rowcolors{1}{}{lightgray}
\resizebox {1\textwidth }{!}{
	\begin{tabular}{lrrl}
    \toprule[1.5pt]
\textbf{ID} &
\textbf{Value} &
\textbf{Cost} &
\textbf{\textit{Dependency Vector} $D_i = \{\sigma_{i,1}\rho_{i,1},...,\sigma_{i,26}\rho_{i,27}\}$}

\\ \midrule

$r_{1}$ &
$10$ &
$5$ &
$\{+0.00,+0.00,+0.00,+0.05,+0.05,+0.00,+0.60,+0.40,+0.00,+0.00,+0.00,+0.20,+0.00,+0.00,+0.00,+0.00,+0.40,+0.00,+0.00,+0.00,+0.05,+0.00,+0.00,+0.90,+0.00,+0.00,+0.00\}$
\\
$r_{2}$ &
$20$ &
$20$ &
$\{+1.00,+0.00,+0.00,+0.60,+0.10,+0.00,+0.60,+0.60,+0.10,+0.30,+0.30,+0.70,+0.00,+0.30,+0.00,+0.40,+0.40,+0.00,+0.00,+0.00,+0.10,+0.00,+0.20,+0.90,+0.00,+1.00,+0.00\}$
\\
$r_{3}$ &
$4$ &
$0$ &
$\{+1.00,+0.00,+0.00,+0.50,+0.10,+0.00,+0.60,+0.00,+0.00,+0.00,+0.00,+0.20,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00\}$
\\
$r_{4}$ &
$17$ &
$10$ &
$\{+0.00,+1.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.40,+0.00,+0.00,+0.20,+0.00,+0.40,+0.00,+0.00,+0.00,+0.00,+0.10,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00\}$
\\
$r_{5}$ &
$3$ &
$1$ &
$\{+1.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.10,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00\}$
\\
$r_{6}$ &
$20$ &
$20$ &
$\{+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.60,+0.00,+0.30,+0.30,+0.40,+0.00,+0.00,+0.00,+0.00,+0.40,+0.40,+0.00,+0.00,+0.00,+0.00,+0.00,+0.30,+0.90,+0.00,+1.00,+0.00\}$
\\
$r_{7}$ &
$15$ &
$6$ &
$\{+0.60,+0.60,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.60,+0.00,+0.00,+0.00\}$
\\
$r_{8}$ &
$9$ &
$5$ &
$\{+1.00,+0.80,+0.00,+0.00,+0.00,+0.80,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+1.00,+0.00,+0.00\}$
\\
$r_{9}$ &
$20$ &
$16$ &
$\{+0.00,+0.50,+0.00,+0.00,+0.00,+1.00,+0.00,+0.30,+0.00,+0.00,+0.80,+0.20,+0.30,+0.00,+0.05,+0.40,+0.00,+0.00,+0.00,+0.00,+0.05,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00\}$
\\
$r_{10}$ &
$16$ &
$10$ &
$\{+0.00,+0.70,+0.00,+0.00,+0.05,+0.70,+0.00,+0.30,+0.00,+0.00,+0.00,+0.00,+0.40,+0.00,+0.00,+0.20,+0.00,+0.00,+0.00,+0.00,+0.10,+0.60,+0.00,+0.00,+0.00,+0.00,+0.00\}$
\\
$r_{11}$ &
$20$ &
$4$ &
$\{+0.00,+0.00,+0.00,+0.40,+0.00,+0.50,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,-0.05,+0.00,+0.00,+0.00,+0.05,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00\}$
\\
$r_{12}$ &
$10$ &
$3$ &
$\{+1.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.80,+0.00,+0.00,+0.00,+0.10,+0.40,+0.00,+0.00,+0.00,+0.00,+0.00,+0.40,+0.00,+0.00,+0.00,+0.00,+0.00\}$
\\
$r_{13}$ &
$6$ &
$5$ &
$\{+0.00,+0.00,+0.00,+0.00,+0.00,+1.00,+0.00,+0.00,+0.00,+0.00,+0.80,+0.00,+0.00,+0.00,+0.10,+0.40,+0.00,+0.00,+0.00,+0.00,+0.00,+0.60,+0.00,+0.00,+0.00,+0.00,+0.00\}$
\\
$r_{14}$ &
$8$ &
$7$ &
$\{+1.00,+0.60,+0.00,+0.00,+0.00,+0.90,+0.00,+0.00,+0.00,+0.00,+0.80,+0.00,+0.00,+0.00,+0.00,+0.80,+0.00,+0.00,+0.00,+0.00,+0.80,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00\}$
\\
$r_{15}$ &
$8$ &
$15$ &
$\{+0.00,+1.00,+0.00,+0.00,+0.00,+0.50,+0.00,+0.00,+0.00,+0.00,+0.20,+0.00,+0.00,+0.00,+0.00,+0.80,+0.00,+0.00,+0.00,+0.00,+1.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00\}$
\\
$r_{16}$ &
$10$ &
$13$ &
$\{+0.00,+1.00,+0.00,+0.00,+0.00,+0.50,+0.00,+0.00,+0.00,+0.00,+0.80,+0.00,+0.00,+0.00,+0.00,+0.00,+0.50,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,-0.02,-0.10\}$
\\
$r_{17}$ &
$6$ &
$14$ &
$\{+1.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.80,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.20,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,-0.05,-0.05\}$
\\
$r_{18}$ &
$10$ &
$3$ &
$\{+1.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+1.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00\}$
\\
$r_{19}$ &
$20$ &
$10$ &
$\{+0.00,+1.00,+0.00,+0.70,+0.50,+1.00,+0.00,+0.50,+1.00,+0.60,+0.40,+0.00,+0.00,+0.10,+0.80,+0.80,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.80,+0.00,+0.00,+0.00,+0.00\}$
\\
$r_{20}$ &
$20$ &
$7$ &
$\{+0.00,+1.00,+0.00,+0.70,+0.50,+1.00,+0.60,+0.50,+1.00,+0.60,+0.40,+0.00,+0.00,+0.10,+0.80,+0.80,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.80,+0.00,+0.00,+0.00,+0.00\}$
\\
$r_{21}$ &
$15$ &
$12$ &
$\{+0.00,+1.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.80,+0.00,+0.00,+0.00,+0.00,+0.80,+0.00,+0.00,+0.00,+0.00,+0.00,+0.30,+0.00,+0.00,+0.00,+0.00,+0.00\}$
\\
$r_{22}$ &
$20$ &
$15$ &
$\{+1.00,+0.00,+0.00,+0.00,+0.00,+0.10,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.10,+0.00,+0.00\}$
\\
$r_{23}$ &
$20$ &
$8$ &
$\{+0.00,+1.00,+0.00,+0.00,+0.00,+0.30,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00\}$
\\
$r_{24}$ &
$5$ &
$2$ &
$\{+1.00,+0.00,+0.00,+0.00,+0.00,+0.10,+0.10,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,-0.01,+0.00,+0.00\}$
\\
$r_{25}$ &
$0$ &
$10$ &
$\{+1.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.80,+0.00,+0.00,+0.00,+0.00\}$
\\
$r_{26}$ &
$0$ &
$0$ &
$\{+1.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+1.00\}$
\\
$r_{27}$ &
$0$ &
$1$ &
$\{+1.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00\}$
\\
$\textbf{Sum}$ &
$\textbf{312}$ &
$\textbf{222}$ &
$$
\\
\bottomrule[1.5pt]
\end{tabular}}%


==> table_cs_dependencies_1.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
%\normalsize\rowcolors{1}{}{lightgray}
\huge\resizebox {1.1\textwidth }{!}{
	\begin{tabular}{lrrlllllllllllllllllllllllllll}
	\toprule[1.5pt]
	\textbf{ID} &
	\textbf{Value} &
	\textbf{Cost} &
	\multicolumn{27}{l}{\boldmath{}\textbf{\textbf{Dependency Vector} $D_i=\{\sigma_{i,1}\rho_{i,1},...,\sigma_{i,27}\rho_{i,27}\}$}\unboldmath{}}
	\\ \midrule
	$r_{1}$ &
	$10$ &
	$5$ &
	$\{\pm 0.00$ ,&
		$\pm 0.00$, &
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.05$ ,&
		\cellcolor{gray!25}$+0.05$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.60$ ,&
		\cellcolor{gray!25}$+0.40$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.20$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.40$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.05$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.90$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00\}$
	\\
	$r_{2}$ &
	$20$ &
	$20$ &
	$\{+1.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.60$ ,&
		\cellcolor{gray!25}$+0.10$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.60$ ,&
		\cellcolor{gray!25}$+0.60$ ,&
		\cellcolor{gray!25}$+0.10$ ,&
		\cellcolor{gray!25}$+0.30$ ,&
		\cellcolor{gray!25}$+0.30$ ,&
		\cellcolor{gray!25}$+0.70$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.30$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.40$ ,&
		\cellcolor{gray!25}$+0.40$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.10$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.20$ ,&
		\cellcolor{gray!25}$+0.90$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+1.00$ ,&
		$\pm 0.00\}$
	\\
	$r_{3}$ &
	$4$ &
	$0$ &
	$\{+1.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.50$ ,&
		\cellcolor{gray!25}$+0.10$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.60$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.20$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00\}$
	\\
	$r_{4}$ &
	$17$ &
	$10$ &
	$\{\pm 0.00$ ,&
		\cellcolor{gray!25}$+1.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.40$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.20$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.40$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.10$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00\}$
	\\
	$r_{5}$ &
	$3$ &
	$1$ &
	$\{+1.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.10$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00\}$
	\\
	$r_{6}$ &
	$20$ &
	$20$ &
	$\{\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.60$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.30$ ,&
		\cellcolor{gray!25}$+0.30$ ,&
		\cellcolor{gray!25}$+0.40$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.40$ ,&
		\cellcolor{gray!25}$+0.40$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.30$ ,&
		\cellcolor{gray!25}$+0.90$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+1.00$ ,&
		$\pm 0.00\}$
	\\
	$r_{7}$ &
	$15$ &
	$6$ &
	$\{+0.60$ ,&
		\cellcolor{gray!25}$+0.60$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.60$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00\}$
	\\
	$r_{8}$ &
	9 &
	5 &
	$\{+1.00$ ,&
		\cellcolor{gray!25}$+0.80$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.80$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+1.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00\}$
	\\
	$r_{9}$ &
	20 &
	16 &
	$\{\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.50$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+1.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.30$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.80$ ,&
		\cellcolor{gray!25}$+0.20$ ,&
		\cellcolor{gray!25}$+0.30$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.05$,&
		\cellcolor{gray!25}$+0.40$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		0.05 ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00\}$
	\\
	$r_{10}$ &
	16 &
	10 &
	$\{\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.70$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.05$ ,&
		\cellcolor{gray!25}$+0.70$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.30$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.40$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.20$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.10$ ,&
		\cellcolor{gray!25}$+0.60$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00\}$
	\\
	$r_{11}$ &
	20 &
	4 &
	$\{\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.40$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.50$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!55}$-0.05$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.05$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00\}$
	\\
	$r_{12}$ &
	10 &
	3 &
	$\{+1.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.80$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.10$ ,&
		\cellcolor{gray!25}$+0.40$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.40$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00\}$
	\\
	$r_{13}$ &
	6 &
	5 &
	$\{\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+1.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.80$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.10$ ,&
		\cellcolor{gray!25}$+0.40$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.60$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00\}$
	\\
	$r_{14}$ &
	8 &
	7 &
	$\{+1.00$ ,&
		\cellcolor{gray!25}$+0.60$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.90$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.80$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.80$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.80$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00\}$
	\\
	$r_{15}$ &
	8 &
	15 &
	$\{\pm 0.00$ ,&
		\cellcolor{gray!25}$+1.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.50$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.20$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.80$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+1.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00\}$
	\\
	$r_{16}$ &
	10 &
	13 &
	$\{\pm 0.00$ ,&
		\cellcolor{gray!25}$+1.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.50$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.80$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.50$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!55}$-0.02$ ,&
		\cellcolor{gray!55}$-0.10\}$
		\\
		$r_{17}$ &
		6 &
		14 &
		$\{+1.00$ ,&
			$\pm 0.00$ ,&
			$\pm 0.00$ ,&
			$\pm 0.00$ ,&
			$\pm 0.00$ ,&
			$\pm 0.00$ ,&
			$\pm 0.00$ ,&
			$\pm 0.00$ ,&
			$\pm 0.00$ ,&
			$\pm 0.00$ ,&
			\cellcolor{gray!25}$+0.80$ ,&
			$\pm 0.00$ ,&
			$\pm 0.00$ ,&
			$\pm 0.00$ ,&
			$\pm 0.00$ ,&
			$\pm 0.00$ ,&
			$\pm 0.00$ ,&
			\cellcolor{gray!25}$+0.20$ ,&
			$\pm 0.00$ ,&
			$\pm 0.00$ ,&
			$\pm 0.00$ ,&
			$\pm 0.00$ ,&
			$\pm 0.00$ ,&
			$\pm 0.00$ ,&
			$\pm 0.00$ ,&
			\cellcolor{gray!55}$-0.05$ ,&
			\cellcolor{gray!55}$-0.05\}$
			\\
			$r_{18}$ &
			10 &
			3 &
			$\{+1.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				\cellcolor{gray!25}$+1.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00\}$
			\\
			$r_{19}$ &
			20 &
			10 &
			$\{\pm 0.00$ ,&
				\cellcolor{gray!25}$+1.00$ ,&
				$\pm 0.00$ ,&
				\cellcolor{gray!25}$+0.70$ ,&
				\cellcolor{gray!25}$+0.50$ ,&
				\cellcolor{gray!25}$+1.00$ ,&
				$\pm 0.00$ ,&
				\cellcolor{gray!25}$+0.50$ ,&
				\cellcolor{gray!25}$+1.00$ ,&
				\cellcolor{gray!25}$+0.60$ ,&
				\cellcolor{gray!25}$+0.40$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				\cellcolor{gray!25}$+0.10$ ,&
				\cellcolor{gray!25}$+0.80$ ,&
				\cellcolor{gray!25}$+0.80$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				\cellcolor{gray!25}$+0.80$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00\}$
			\\
			$r_{20}$ &
			20 &
			7 &
			$\{\pm 0.00$ ,&
				\cellcolor{gray!25}$+1.00$ ,&
				$\pm 0.00$,&
				\cellcolor{gray!25}$+0.70$ ,&
				\cellcolor{gray!25}$+0.50$ ,&
				\cellcolor{gray!25}$+1.00$ ,&
				\cellcolor{gray!25}$+0.60$ ,&
				\cellcolor{gray!25}$+0.50$ ,&
				\cellcolor{gray!25}$+1.00$ ,&
				\cellcolor{gray!25}$+0.60$ ,&
				\cellcolor{gray!25}$+0.40$ ,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				\cellcolor{gray!25}$+0.10$ ,&
				\cellcolor{gray!25}$+0.80$ ,&
				\cellcolor{gray!25}$+0.80$ ,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				\cellcolor{gray!25}$+0.80$ ,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00\}$
			\\
			$r_{21}$ &
			15 &
			12 &
			$\{\pm 0.00$ ,&
				\cellcolor{gray!25}$+1.00$ ,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				\cellcolor{gray!25}$+0.80$ ,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				\cellcolor{gray!25}$+0.80$ ,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				\cellcolor{gray!25}$+0.30$ ,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00\}$
			\\
			$r_{22}$ &
			20 &
			15 &
			$\{+1.00$ ,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				\cellcolor{gray!25}$+0.10$ ,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				\cellcolor{gray!25}$+0.10$ ,&
				$\pm 0.00$,&
				$\pm 0.00\}$
			\\
			$r_{23}$ &
			20 &
			8 &
			$\{\pm 0.00$ ,&
				\cellcolor{gray!25}$+1.00$ ,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				\cellcolor{gray!25}$+0.30$ ,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00\}$
			\\
			$r_{24}$ &
			5 &
			2 &
			$\{+1.00$ &
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				\cellcolor{gray!25}$+0.10$ ,&
				\cellcolor{gray!25}$+0.10$ ,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				\cellcolor{gray!55}$-0.01$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00\}$
			\\
			$r_{25}$ &
			$0$ &
			$10$ &
			$\{+1.00$ &
				$\pm 0.00$ ,& 
				$\pm 0.00$ ,& 
				$\pm 0.00$ ,& 
				$\pm 0.00$ ,& 
				$\pm 0.00$ ,& 
				$\pm 0.00$ ,& 
				$\pm 0.00$ ,& 
				$\pm 0.00$ ,& 
				$\pm 0.00$ ,& 
				$\pm 0.00$ ,& 
				$\pm 0.00$ ,& 
				$\pm 0.00$ ,& 
				$\pm 0.00$ ,& 
				$\pm 0.00$ ,& 
				$\pm 0.00$ ,& 
				$\pm 0.00$ ,& 
				$\pm 0.00$ ,& 
				$\pm 0.00$ ,& 
				$\pm 0.00$ ,& 
				$\pm 0.00$ ,& 
				$\pm 0.00$ ,& 
				\cellcolor{gray!25}$+0.80$ ,&
				$\pm 0.00$ ,& 
				$\pm 0.00$ ,& 
				$\pm 0.00$ ,& 
				$\pm 0.00\}$
			\\
			$r_{26}$ &
			$0$ & 
			$0$  &
			$\{+1.00$ ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00\}$
			\\
			$r_{27}$ &
			$0$  &
			$1$ &
			$\{+1.00$ ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00\}$
				\\ \midrule
				$\textbf{Sum}$ &
				$\textbf{312}$ &
				$\textbf{222}$ &
				$$
			\\	\toprule[1.5pt]
		\end{tabular}}%


==> table_cs_solutions.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
%\rowcolors{1}{}{lightgray}
\resizebox {0.8\textwidth }{!}{% Table generated by Excel2LaTeX from sheet 'Sheet6'
	\begin{tabular}{llll}
		\toprule[1.5pt]
		\textbf{Budget (relative)} &
		\textbf{Selection Model} &
		\textbf{Overall Value (percent)} &
		\boldmath{}\textbf{Solution Vector ($r_1,...,r_{23}$)}\unboldmath{}
		\\ \midrule[1.5pt]
		\multirow{3}[1]{*}{16} &
		BKP &
		5.21 &
		$\{0,1,1,0,0,0,0,0,0,0,1,0,0,0,0,1,0,0,0,0,0,0,0\}$
		\\
		&
		BKP-PC &
		10.74 &
		$\{0,0,0,0,0,0,1,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,1\}$
		\\
		&
		GORS &
		12.88 &
		$\{0,0,0,0,0,0,1,0,0,0,1,0,0,0,0,1,0,1,0,0,0,0,0\}$
		\bigstrut[b]\\
		\hline
		\multirow{3}[2]{*}{46} &
		BKP &
		23.25 &
		$\{1,1,1,0,0,0,1,0,0,0,1,0,0,0,0,1,0,1,0,0,0,0,1\}$
		\bigstrut[t]\\
		&
		BKP-PC &
		19.94 &
		$\{0,0,0,0,0,0,1,0,0,0,0,0,0,0,0,0,0,1,0,0,0,1,1\}$
		\\
		&
		GORS &
		26.63 &
		$\{0,0,0,0,0,0,1,0,0,0,1,0,1,0,0,1,0,1,0,0,0,1,1\}$
		\bigstrut[b]\\
		\hline
		\multirow{3}[2]{*}{71} &
		BKP &
		31.07 &
		$\{1,1,1,1,0,0,1,0,0,1,1,1,0,0,0,1,0,1,0,0,0,0,1\}$
		\bigstrut[t]\\
		&
		BKP-PC &
		19.94 &
		$\{0,0,0,0,0,0,1,0,0,0,0,0,0,0,0,0,0,1,0,0,0,1,1\}$
		\\
		&
		GORS &
		34.60 &
		$\{1,1,1,0,0,0,1,0,0,0,1,1,1,0,0,1,0,1,0,0,0,1,1\}$
		\bigstrut[b]\\
		\hline
		\multirow{3}[2]{*}{76} &
		BKP &
		32.06 &
		$\{1,1,1,1,0,0,1,0,0,1,1,1,1,0,0,1,0,1,0,0,0,0,1\}$
		\bigstrut[t]\\
		&
		BKP-PC &
		19.94 &
		$\{0,0,0,0,0,0,1,0,0,0,0,0,0,0,0,0,0,1,0,0,0,1,1\}$
		\\
		&
		GORS &
		35.74 &
		$\{1,1,1,1,0,0,1,0,0,0,1,1,0,0,0,1,0,1,0,0,0,1,1\}$
		\bigstrut[b]\\
		\hline
		\multirow{3}[2]{*}{81} &
		BKP &
		31.90 &
		$\{1,1,1,1,0,0,1,0,0,1,1,0,1,0,0,1,1,1,0,0,0,0,1\}$
		\bigstrut[t]\\
		&
		BKP-PC &
		19.94 &
		$\{0,0,0,0,0,0,1,0,0,0,0,0,0,0,0,0,0,1,0,0,0,1,1\}$
		\\
		&
		GORS &
		37.98 &
		$\{0,0,0,1,0,0,0,0,0,0,1,0,0,1,0,1,1,1,0,0,1,1,1\}$
		\bigstrut[b]\\
		\hline
		\multirow{3}[2]{*}{141} &
		BKP &
		44.11 &
		$\{1,1,1,1,0,0,1,0,1,1,1,1,1,0,0,1,1,1,0,1,0,1,1\}$
		\bigstrut[t]\\
		&
		BKP-PC &
		53.37 &
		$\{0,0,0,1,1,0,1,1,0,0,1,0,1,1,1,1,1,1,0,0,1,1,1\}$
		\\
		&
		GORS &
		59.45 &
		$\{1,1,1,1,0,0,1,0,0,1,1,1,1,1,1,1,1,1,0,0,1,1,1\}$
		\bigstrut[b]\\
		\hline
		\multirow{3}[2]{*}{146} &
		BKP &
		45.40 &
		$\{1,1,1,1,0,0,1,0,1,1,1,1,0,0,0,1,1,1,0,1,1,1,1\}$
		\bigstrut[t]\\
		&
		BKP-PC &
		53.37 &
		$\{0,0,0,1,1,0,1,1,0,0,1,0,1,1,1,1,1,1,0,0,1,1,1\}$
		\\
		&
		GORS &
		60.43 &
		$\{1,1,1,1,0,0,1,1,0,0,1,1,1,1,1,1,1,1,0,0,1,1,1\}$
		\bigstrut[b]\\
		\hline
		\multirow{3}[2]{*}{151} &
		BKP &
		46.87 &
		$\{1,1,1,1,0,0,1,0,1,1,1,1,1,0,0,1,1,1,0,1,1,1,1\}$
		\bigstrut[t]\\
		&
		BKP-PC &
		53.37 &
		$\{0,0,0,1,1,0,1,1,0,0,1,0,1,1,1,1,1,1,0,0,1,1,1\}$
		\\
		&
		GORS &
		62.27 &
		$\{1,1,1,1,0,1,1,0,0,0,1,1,1,1,1,1,1,1,0,0,1,1,1\}$
		\bigstrut[b]\\
		\hline
		\multirow{3}[2]{*}{156} &
		BKP &
		46.87 &
		$\{1,1,1,1,0,0,1,0,1,1,1,1,1,0,0,1,1,1,0,1,1,1,1\}$
		\bigstrut[t]\\
		&
		BKP-PC &
		53.37 &
		$\{0,0,0,1,1,0,1,1,0,0,1,0,1,1,1,1,1,1,0,0,1,1,1\}$
		\\
		&
		GORS &
		62.27 &
		$\{1,1,1,1,0,1,1,0,0,0,1,1,1,1,1,1,1,1,0,0,1,1,1\}$
		\bigstrut[b]\\
		\hline
		\multirow{3}[2]{*}{161} &
		BKP &
		50.12 &
		$\{1,1,1,1,0,1,1,0,1,1,1,1,1,0,0,1,1,1,0,1,0,1,1\}$
		\bigstrut[t]\\
		&
		BKP-PC &
		53.37 &
		$\{0,0,0,1,1,0,1,1,0,0,1,0,1,1,1,1,1,1,0,0,1,1,1\}$
		\\
		&
		GORS &
		64.23 &
		$\{1,1,1,1,0,1,1,0,0,1,1,1,1,1,1,1,1,1,0,0,1,1,1\}$
		\bigstrut[b]\\
		\hline
		\multirow{3}[2]{*}{166} &
		BKP &
		51.41 &
		$\{1,1,1,1,0,1,1,0,1,1,1,1,0,0,0,1,1,1,0,1,1,1,1\}$
		\bigstrut[t]\\
		&
		BKP-PC &
		53.37 &
		$\{0,0,0,1,1,0,1,1,0,0,1,0,1,1,1,1,1,1,0,0,1,1,1\}$
		\\
		&
		GORS &
		64.72 &
		$\{1,1,1,1,0,1,1,0,1,0,1,1,1,1,1,1,1,1,0,0,1,1,1\}$
		\bigstrut[b]\\
		\hline
		\multirow{3}[2]{*}{171} &
		BKP &
		52.88 &
		$\{1,1,1,1,0,1,1,0,1,1,1,1,1,0,0,1,1,1,0,1,1,1,1\}$
		\bigstrut[t]\\
		&
		BKP-PC &
		53.37 &
		$\{0,0,0,1,1,0,1,1,0,0,1,0,1,1,1,1,1,1,0,0,1,1,1\}$
		\\
		&
		GORS &
		64.72 &
		$\{1,1,1,1,0,1,1,0,1,0,1,1,1,1,1,1,1,1,0,0,1,1,1\}$
		\bigstrut[b]\\
		\hline
		\multirow{3}[2]{*}{176} &
		BKP &
		52.88 &
		$\{1,1,1,1,0,1,1,0,1,1,1,1,1,0,0,1,1,1,0,1,1,1,1\}$
		\bigstrut[t]\\
		&
		BKP-PC &
		53.37 &
		$\{0,0,0,1,1,0,1,1,0,0,1,0,1,1,1,1,1,1,0,0,1,1,1\}$
		\\
		&
		GORS &
		66.69 &
		$\{1,1,1,1,0,1,1,1,0,1,1,1,1,1,1,1,1,1,0,0,1,1,1\}$
		\bigstrut[b]\\
		\hline
		\multirow{3}[2]{*}{181} &
		BKP &
		51.35 &
		$\{1,1,1,1,0,1,1,0,1,1,1,1,1,0,0,1,1,1,1,1,0,1,1\}$
		\bigstrut[t]\\
		&
		BKP-PC &
		53.37 &
		$\{0,0,0,1,1,0,1,1,0,0,1,0,1,1,1,1,1,1,0,0,1,1,1\}$
		\\
		&
		GORS &
		67.18 &
		$\{1,1,1,1,0,1,1,1,1,0,1,1,1,1,1,1,1,1,0,0,1,1,1\}$
		\bigstrut[b]\\
		\hline
		\multirow{3}[2]{*}{186} &
		BKP &
		52.64 &
		$\{1,1,1,1,0,1,1,0,1,1,1,1,0,0,0,1,1,1,1,1,1,1,1\}$
		\bigstrut[t]\\
		&
		BKP-PC &
		53.37 &
		$\{0,0,0,1,1,0,1,1,0,0,1,0,1,1,1,1,1,1,0,0,1,1,1\}$
		\\
		&
		GORS &
		73.83 &
		$\{1,1,0,1,1,1,1,1,1,1,1,1,1,1,0,1,1,1,0,0,1,1,1\}$
		\bigstrut[b]\\
		\hline
		\multirow{3}[2]{*}{191} &
		BKP &
		54.11 &
		$\{1,1,1,1,0,1,1,0,1,1,1,1,1,0,0,1,1,1,1,1,1,1,1\}$
		\bigstrut[t]\\
		&
		BKP-PC &
		53.37 &
		$\{0,0,0,1,1,0,1,1,0,0,1,0,1,1,1,1,1,1,0,0,1,1,1\}$
		\\
		&
		GORS &
		75.31 &
		$\{1,1,1,1,1,1,1,1,1,1,1,1,1,1,0,1,1,1,0,0,1,1,1\}$
		\bigstrut[b]\\
		\hline
		\multirow{3}[2]{*}{196} &
		BKP &
		54.11 &
		$\{1,1,1,1,0,1,1,0,1,1,1,1,1,0,0,1,1,1,1,1,1,1,1\}$
		\bigstrut[t]\\
		&
		BKP-PC &
		53.37 &
		$\{0,0,0,1,1,0,1,1,0,0,1,0,1,1,1,1,1,1,0,0,1,1,1\}$
		\\
		&
		GORS &
		75.31 &
		$\{1,1,1,1,1,1,1,1,1,1,1,1,1,1,0,1,1,1,0,0,1,1,1\}$
		\bigstrut[b]\\
		\hline
		\multirow{3}[1]{*}{246} &
		BKP &
		100.00 &
		$\{1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1\}$
		\bigstrut[t]\\
		&
		BKP-PC &
		100.00 &
		$\{1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1\}$
		\\
		&
		GORS &
		100.00 &
		$\{1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1\}$
		\\ \bottomrule[1.5pt]
	\end{tabular}}%


==> table_data.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\resizebox {0.7\textwidth}{!}{
\begin{tabular}{| r | r | r | r |  r| r |  r | r | r | r | r | r | r | r | r | r |}
\Xhline{4\arrayrulewidth}
 &
  Requirement &
  $r_0$ &
  $r_1$ &
  $r_2$ &
  $r_3$ &
  $r_4$ &
  $r_5$ &
  $r_6$ &
  $r_7$ &
  $r_8$ &
  $r_9$ &
  $r_{10}$ &
  $r_{11}$ &
  $r_{12}$ &
  $r_{13}$
  \bigstrut\\
\hline
\multirow{2}[4]{*}{\textbf{RAN}} &
  Value &
  $12$ &
  $6$ &
  $5$ &
  $7$ &
  $12$ &
  $16$ &
  $3$ &
  $3$ &
  $4$ &
  $5$ &
  $1$ &
  $1$ &
  $21$ &
  $3$
  \bigstrut\\
\cline{2-16} &
  Cost &
  $1$ &
  $2$ &
  $3$ &
  $4$ &
  $6$ &
  $11$ &
  $4$ &
  $6$ &
  $7$ &
  $12$ &
  $4$ &
  $6$ &
  $23$ &
  $10$
  \bigstrut\\
\hline
\multirow{2}[4]{*}{\textbf{PMR}} &
  Value &
  $0$ &
  $6$ &
  $3$ &
  $11$ &
  $32$ &
  $20$ &
  $9$ &
  $4$ &
  $25$ &
  $9$ &
  $3$ &
  $\--$ &
  $\--$ &
  $\--$ 
  \bigstrut\\
\cline{2-16} &
  Cost &
  $6$ &
  $5$ &
  $6$ &
  $19$ &
  $28$ &
  $4$ &
  $5$ &
  $7$ &
  $10$ &
  $3$ &
  $8$ &
  $\--$ &
  $\--$ &
  $\--$ 
  \bigstrut\\
\Xhline{4\arrayrulewidth}
\end{tabular}
}%



==> table_ex_all.tex <==
%\rowcolor{lightgray}
\rowcolors{1}{}{lightgray}
\resizebox {0.7\textwidth }{!}{% Table generated by Excel2LaTeX from sheet 'allsolution_requirements_0.125'
% Table generated by Excel2LaTeX from sheet 'allsolution_requirements_0.125'
% Table generated by Excel2LaTeX from sheet 'allsolution_requirements_0.125'
% Table generated by Excel2LaTeX from sheet 'allsolution_requirements_0.125'
\begin{tabular}{llccc}
	\toprule[1.5pt]
	$X_k=$$\{ x_{0},x_{1},x_{2},x_{3} \}$ &
	$P_k=$$\{ p_{0},p_{1},p_{2},p_{3} \}$ &
	$AC=\displaystyle \sum_{i=1}^{n} x_i c_i$ &
	$ACV=\displaystyle \sum_{i=1}^{n} x_iv_i$ &
	$OCV=\displaystyle \sum_{i=1}^{n} x_i (v_i - p_iv_i)$
	\\ \midrule
	$X_{0}=\{0,0,0,0\}$ &
	$P_{0}=\{0.0,0.0,0.0,0.0\}$ &
	$0.0$ &
	$0.0$ &
	$0.0$
	\\
	$X_{1}=\{1,0,0,0\}$ &
	$P_{1}=\{0.7,0.0,0.0,0.0\}$ &
	$10.0$ &
	$20.0$ &
	$6.0$
	\\
	$X_{2}=\{0,1,0,0\}$ &
	$P_{2}=\{0.0,0.3,0.0,0.0\}$ &
	$10.0$ &
	$10.0$ &
	$7.0$
	\\
	$X_{3}=\{1,1,0,0\}$ &
	$P_{3}=\{0.7,0.3,0.0,0.0\}$ &
	$20.0$ &
	$30.0$ &
	$13.0$
	\\
	$X_{4}=\{0,0,1,0\}$ &
	$P_{4}=\{0.0,0.0,0.7,0.0\}$ &
	$15.0$ &
	$50.0$ &
	$15.0$
	\\
	$X_{5}=\{1,0,1,0\}$ &
	$P_{5}=\{0.7,0.0,0.7,0.0\}$ &
	$25.0$ &
	$70.0$ &
	$21.0$
	\\
	$X_{6}=\{0,1,1,0\}$ &
	$P_{6}=\{0.0,0.3,0.7,0.0\}$ &
	$25.0$ &
	$60.0$ &
	$22.0$
	\\
	$X_{7}=\{1,1,1,0\}$ &
	$P_{7}=\{0.7,0.3,0.7,0.0\}$ &
	$35.0$ &
	$80.0$ &
	$28.0$
	\\
	$X_{8}=\{0,0,0,1\}$ &
	$P_{8}=\{0.0,0.0,0.0,0.2\}$ &
	$10.0$ &
	$10.0$ &
	$8.0$
	\\
	$X_{9}=\{1,0,0,1\}$ &
	$P_{9}=\{0.7,0.0,0.0,0.2\}$ &
	$20.0$ &
	$30.0$ &
	$14.0$
	\\
	$X_{10}=\{0,1,0,1\}$ &
	$P_{10}=\{0.0,0.2,0.0,0.2\}$ &
	$20.0$ &
	$20.0$ &
	$16.0$
	\\
	$X_{11}=\{1,1,0,1\}$ &
	$P_{11}=\{0.7,0.2,0.0,0.2\}$ &
	$30.0$ &
	$40.0$ &
	$22.0$
	\\
	$X_{12}=\{0,0,1,1\}$ &
	$P_{12}=\{0.0,0.0,0.6,0.2\}$ &
	$25.0$ &
	$60.0$ &
	$28.0$
	\\
	$X_{13}=\{1,0,1,1\}$ &
	$P_{13}=\{0.5,0.0,0.5,0.2\}$ &
	$35.0$ &
	$80.0$ &
	$43.0$
	\\
	$X_{14}=\{0,1,1,1\}$ &
	$P_{14}=\{0.0,0.2,0.6,0.2\}$ &
	$35.0$ &
	$70.0$ &
	$36.0$
	\\
	$X_{15}=\{1,1,1,1\}$ &
	$P_{15}=\{0.0,0.0,0.0,0.0\}$ &
	$45.0$ &
	$90.0$ &
	$90.0$
	\\ \bottomrule[1.5pt]
\end{tabular}
}





==> table_ex_all_2.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet5'
\resizebox {1\textwidth }{!}{\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
	\Xhline{4\arrayrulewidth}
$\textbf{Solution}$ &
  $S_0$ &
  $S_1$ &
  $S_2$ &
  $S_3$ &
  $S_4$ &
  $S_5$ &
  $S_6$ &
  $S_7$ &
  $S_8$ &
  $S_9$ &
  $S_{10}$ &
  $S_{11}$ &
  $S_{12}$ &
  $S_{13}$ &
  $S_{14}$ &
  $S_{15}$
  \bigstrut\\
\hline
$\textbf{O}$ &
  $\{\}$ &
  $\{r_1\}$ &
  $\{r_2\}$ &
  $\{r_3\}$ &
  $\{r_4\}$ &
  $\{r1_,r_2\}$ &
  $\{r_1,r_3\}$ &
  $\{r_2,r_4\}$ &
  $\{r_2,r_3\}$ &
  $\{r_2,r_4\}$ &
  $\{r_3,r_4\}$ &
  $\{r_1,r_2,r_3\}$ &
  $\{r_1,r_2,r_4\}$ &
  $\{r_1,r_3,r_4\}$ &
  $\{r_2,r_3,r_4\}$ &
  $\{r_1,r_2,r_3,r_4\}$
  \bigstrut\\
\hline
$\tilde{\textbf{O}}$ &
  $\{r_1,r_2,r_3,r_4\}$ &
  $\{r_2,r_3,r_4\}$ &
	$\{r_1,r_3,r_4\}$ &
  $\{r_1,r_2,r_4\}$ &
  $\{r_1,r_2,r_3\}$ &
  $\{r_3,r_4\}$ &
  $\{r_2,r_4\}$ &
  $\{r_2,r_3\}$ &
  $\{r_2,r_4\}$ &
  $\{r_1,r_3\}$ &
  $\{r1_,r_2\}$ &
  $\{r_4\}$ &
  $\{r_3\}$ &
  $\{r_2\}$ &
  $\{r_1\}$ &
	$\{\}$ 

  \bigstrut\\
\hline
$\textbf{AC}$ &
  $0$ &
  $10$ &
  $10$ &
  $15$ &
  $10$ &
  $20$ &
  $25$ &
  $20$ &
  $25$ &
  $20$ &
  $25$ &
  $35$ &
  $30$ &
  $35$ &
  $35$ &
  $45$
  \bigstrut\\
\hline
$\textbf{AV}$ &
  $0$ &
  $20$ &
  $10$ &
  $50$ &
  $10$ &
  $30$ &
  $70$ &
  $30$ &
  $60$ &
  $20$ &
  $60$ &
  $80$ &
  $40$ &
  $80$ &
  $70$ &
  $90$
  \bigstrut\\
\hline
$\textbf{OV}$ &
  $0$ &
  $4$ &
  $8$ &
  $15$ &
  $8$ &
  $12$ &
  $21$ &
  $12$ &
  $23$ &
  $16$ &
  $23$ &
  $29$ &
  $20$ &
  $36$ &
  $31$ &
	$90$ 
  \bigstrut\\
	\Xhline{4\arrayrulewidth}
\end{tabular}}

==> table_ex_constraints.tex <==
\rowcolors{1}{}{lightgray}
\resizebox {0.4\textwidth }{!}{\begin{tabular}{ccccccccc}
  \toprule[1.5pt]
  \head{} & \head{$x_1$} & \head{$x_2$} & \head{$x_3$} & \head{$x_4$} & \head{$1-x_1$} & \head{$1-x_2$} & \head{$1-x_3$} & \head{$1-x_4$} \\
  %\midrule
	\Xhline{3\arrayrulewidth}
  $x_1$ & $-$ & $\leq$ & $\leq$ & $\leq$ &  $-$ & $\leq$ & $\leq$ & $\leq$ \\
  $x_2$ & $\leq$ & $-$ & $\leq$ & $\leq$ &  $-$ & $-$ & $-$ & $-$ \\
  $x_3$ & $\leq$ & $\leq$ & $-$ & $\leq$ &  $-$ & $-$ & $-$ & $\leq$ \\
  $x_4$ & $-$ & $\leq$ & $\leq$ & $-$    &  $-$ & $-$ & $-$ & $-$ \\

  \bottomrule[1.5pt]
\end{tabular}}



==> table_ex_overall_influence.tex <==
\rowcolors{1}{}{lightgray}
\resizebox {0.9\textwidth }{!}{\begin{tabular}{cccccc}
  \toprule[1.5pt]
  \head{$OI_{i,j}=\rho_{i,j}^{+\infty}-\rho_{i,j}^{-\infty}$} & \head{$r_1$} & \head{$r_2$} & \head{$r_3$} & \head{$r_4$} & \head{$r_5$}\\
  %\midrule
	\Xhline{3\arrayrulewidth}
  $r_1$ & $0.0-0.0=0.0$ & $0.4-0.0=0.0$ & $0.2-0.3=-0.1$ & $0.3-0.0=0.3$ & $0.0-0.5=-0.5$\\
  $r_2$ & $0.0-0.0=0.0$ & $0.0-0.0=0.0$ & $0.2-0.0=0.2$ & $0.0-0.0=0.0$ & $0.0-0.0=0.0$ \\
  $r_3$ & $0.0-0.0=0.0$ & $0.0-0.0=0.0$ & $0.0-0.0=0.0$ & $0.0-0.0=0.0$ & $0.0-0.0=0.0$ \\
  $r_4$ & $0.0-0.0=0.0$ & $0.0-0.0=0.0$ & $0.0-0.0=0.0$ & $0.0-0.0=0.0$ & $0.0-0.0=0.0$ \\
  $r_5$ & $0.0-0.0=0.0$ & $0.0-0.0=0.0$ & $0.0-0.0=0.0$ & $0.0-0.0=0.0$ & $0.0-0.0=0.0$ \\
  \bottomrule[1.5pt]
\end{tabular}}



==> table_ex_overall_strengths.tex <==
\rowcolors{1}{}{lightgray}
\resizebox {0.7\textwidth }{!}{\begin{tabular}{cccccc}
  \toprule[1.5pt]
  \head{$OI_{i,j}=\rho_{i,j}^{+\infty}-\rho_{i,j}^{-\infty}$} & \head{$r_1$} & \head{$r_2$} & \head{$r_3$} & \head{$r_4$} & \head{$r_5$}\\
  %\midrule
	\Xhline{3\arrayrulewidth}
  $r_1$ & $0.0/0.0$ & $0.4/0.0$ & $0.2/0.3$ & $0.3/0.0$ & $0.0/0.5$\\
  $r_2$ & $0.0/0.0$ & $0.0/0.0$ & $0.2/0.0$ & $0.0/0.0$ & $0.0/0.0$ \\
  $r_3$ & $0.0/0.0$ & $0.0/0.0$ & $0.0/0.0$ & $0.0$ & $0.0/0.0$ \\
  $r_4$ & $0.0/0.0$ & $0.0/0.0$ & $0.0/0.0$ & $0.0/0.0$ & $0.0/0.0$ \\
  $r_5$ & $0.0/0.0$ & $0.0/0.0$ & $0.0/0.0$ & $0.0/0.0$ & $0.0/0.0$ \\
  \bottomrule[1.5pt]
\end{tabular}}



==> table_lr.tex <==
\LARGE
%\rowcolors{1}{}{lightmyblue}
\resizebox {0.8\textwidth }{!}{% Table generated by Excel2LaTeX from sheet 'Sheet1'
% Table generated by Excel2LaTeX from sheet 'Sheet1'
% Table generated by Excel2LaTeX from sheet 'Sheet4'
\begin{tabular}{l|l|lllllll}
	\toprule[1.5pt]
	\textbf{\cellcolor{header}\textcolor{white}{Employed Model}}&
	\textbf{\cellcolor{header}\textcolor{white}{Works from the Literature}} &
	\textbf{\cellcolor{header}\textcolor{white}{P1}} &
	\textbf{\cellcolor{header}\textcolor{white}{P2}} &
	\textbf{\cellcolor{header}\textcolor{white}{P3}} &
	\textbf{\cellcolor{header}\textcolor{white}{P4}} &
	\textbf{\cellcolor{header}\textcolor{white}{P5}} &
	\textbf{\cellcolor{header}\textcolor{white}{P6}} &
	\textbf{\cellcolor{header}\textcolor{white}{P7}}
	\\\midrule[1.5pt]
	\multicolumn{1}{l|}{\cellcolor{myblue!30}BKP} 
	\cellcolor{myblue!30}&\begin{tabular}[t]{@{}c@{}} \cite{karlsson_optimizing_1997,jung_optimizing_1998,zhang_multi_objective_2007,baker_search_2006,finkelstein2009search,zhang2011comparing,del2010ant,kumari2012software} \phantom{sssssssssssss} \end{tabular} &
	\cellcolor{myblue!30}NO &
	\cellcolor{myblue!30}NO &
	\cellcolor{myblue!30}NO &
	\cellcolor{myblue!30}NO &
	\cellcolor{myblue!30}NO &
	\cellcolor{myblue!30}NO &
	\cellcolor{myblue!30}NO
	\\ 
	\multicolumn{1}{l|}{\cellcolor{myblue!20}BKP-PC} &
	{1}\cellcolor{myblue!20}\begin{tabular}[t]{@{}c@{}} \cite{veerapen2015integer,brasil_multiobjective_2012,bagnall_next_2001,greer_software_2004,boschetti_lagrangian_2014,ruhe_quantitative_2003,van2011quantitative,zhang2010search,tonella2010using,freitas2011software}\\\cite{colares_new_2009,saliu2007bi,saliu2005supporting,jiang2010hybrid,van2005determination,ngo2009optimized,chen2013ant,del2011requirements,araujo2016architecture,colares2009new,pitangueira2016risk}\end{tabular}  &
	\cellcolor{myblue!20}YES &
	\cellcolor{myblue!20}YES &
	\cellcolor{myblue!20}NO &
	\cellcolor{myblue!20}NO &
	\cellcolor{myblue!20}NO &
	\cellcolor{myblue!20}YES &
	\cellcolor{myblue!20}NO
	\\
	\multicolumn{1}{l|}{\cellcolor{myblue!20}} &
	\cellcolor{myblue!20}\cite{van2008software,ngo_wicked_2008} &
	\cellcolor{myblue!20}YES &
	\cellcolor{myblue!20}YES &
	\cellcolor{myblue!20}YES &
	\cellcolor{myblue!20}NO &
	\cellcolor{myblue!20}NO &
	\cellcolor{myblue!20}YES &
	\cellcolor{myblue!20}NO
	\\
	\multicolumn{1}{l|}{\cellcolor{myblue!20}} &
	\cellcolor{myblue!20}\cite{tonella2013interactive,xuan2012solving,saliu2005software} &
	\cellcolor{myblue!20}YES &
	\cellcolor{myblue!20}NO &
	\cellcolor{myblue!20}NO &
	\cellcolor{myblue!20}NO &
	\cellcolor{myblue!20}NO &
	\cellcolor{myblue!20}YES &
	\cellcolor{myblue!20}NO
	\\
	\multicolumn{1}{l|}{\cellcolor{myblue!20}} &
	\cellcolor{myblue!20}\cite{li2016value} &
	\cellcolor{myblue!20}NO &
	\cellcolor{myblue!20}NO &
	\cellcolor{myblue!20}NO &
	\cellcolor{myblue!20}NO &
	\cellcolor{myblue!20}NO &
	\cellcolor{myblue!20}YES &
	\cellcolor{myblue!20}NO
	\\
	\multicolumn{1}{l|}{\cellcolor{myblue!10}Increase/Decrease\_Value\_Of} &
	\cellcolor{myblue!10}\cite{li_integrated_2010,sagrado_multi_objective_2013,Zhang_RIM_2013} (Subsets of Size 2)&
	\cellcolor{myblue!10}YES &
	\cellcolor{myblue!10}NO &
	\cellcolor{myblue!10}YES &
	\cellcolor{myblue!10}YES &
	\cellcolor{myblue!10}NO &
	\cellcolor{myblue!10}YES &
	\cellcolor{myblue!10}YES
	\\
	\multicolumn{1}{l|}{\cellcolor{myblue!10}} &
	\cellcolor{myblue!10}\cite{van_den_akker_flexible_2005} (Subsets of Any Size)&
	\cellcolor{myblue!10}YES &
	\cellcolor{myblue!10}YES &
	\cellcolor{myblue!10}NO &
	\cellcolor{myblue!10}NO &
	\cellcolor{myblue!10}NO &
	\cellcolor{myblue!10}YES &
	\cellcolor{myblue!10}YES
	\\\bottomrule[1.5pt]
\end{tabular}
}




==> table_lr1.tex <==
\LARGE
%\rowcolors{1}{}{lightmyblue}
\resizebox {0.9\textwidth }{!}{% Table generated by Excel2LaTeX from sheet 'Sheet1'
	% Table generated by Excel2LaTeX from sheet 'Sheet1'
	% Table generated by Excel2LaTeX from sheet 'Sheet4'
	% Table generated by Excel2LaTeX from sheet 'Sheet1'
	\begin{tabular}{l|l|lllllll}
		\hline
		\textbf{\cellcolor{header}\textcolor{white}{Employed Model}} &
		\textbf{\cellcolor{header}\textcolor{white}{Works}} &
		\textbf{\cellcolor{header}\textcolor{white}{P1}} &
		\textbf{\cellcolor{header}\textcolor{white}{P2}} &
		\textbf{\cellcolor{header}\textcolor{white}{P3}} &
		\textbf{\cellcolor{header}\textcolor{white}{P4}} &
		\textbf{\cellcolor{header}\textcolor{white}{P5}} &
		\textbf{\cellcolor{header}\textcolor{white}{P6}} &
		\textbf{\cellcolor{header}\textcolor{white}{P7}}
		\bigstrut\\
		\hline
		\cellcolor{myblue!30} BKP & 
		\cellcolor{myblue!30}\begin{tabular}[t]{@{}c@{}} \cite{karlsson_optimizing_1997,jung_optimizing_1998,zhang_multi_objective_2007,baker_search_2006,finkelstein2009search,zhang2011comparing,del2010ant,kumari2012software} \phantom{sssssssssssss} \end{tabular}&
		\cellcolor{myblue!30}NO &
		\cellcolor{myblue!30}NO &
		\cellcolor{myblue!30}NO &
		\cellcolor{myblue!30}NO &
		\cellcolor{myblue!30}NO &
		\cellcolor{myblue!30}NO &
		\cellcolor{myblue!30}NO
		
		\bigstrut\\
		\hline
		\multirow{4}[10]{*}{BKP-PC} &
		\cellcolor{myblue!20}\begin{tabular}[t]{@{}c@{}} \cite{veerapen2015integer,brasil_multiobjective_2012,sagrado_multi_objective_2013,bagnall_next_2001,greer_software_2004,boschetti_lagrangian_2014,ruhe_quantitative_2003,van2011quantitative,zhang2010search,tonella2010using,freitas2011software}\\ \cellcolor{myblue!20}\cite{colares_new_2009,saliu2007bi,saliu2005supporting,jiang2010hybrid,van2005determination,ngo2009optimized,chen2013ant,del2011requirements,araujo2016architecture,colares2009new,pitangueira2016risk}\end{tabular}  &
		\cellcolor{myblue!20}YES &
		\cellcolor{myblue!20}YES &
		\cellcolor{myblue!20}NO  &
		\cellcolor{myblue!20}NO  &
		\cellcolor{myblue!20}NO  &
		\cellcolor{myblue!20}YES &
		\cellcolor{myblue!20}NO
		
		\bigstrut\\
		\cline{2-9}  & 
		
		\cellcolor{myblue!20}\cite{van2008software,ngo_wicked_2008} &
		\cellcolor{myblue!20}YES &
		\cellcolor{myblue!20}YES &
		\cellcolor{myblue!20}YES &
		\cellcolor{myblue!20}NO &
		\cellcolor{myblue!20}NO &
		\cellcolor{myblue!20}YES &
		\cellcolor{myblue!20}NO
		
		\bigstrut\\
		\cline{2-9} & 
		
		\cellcolor{myblue!20}\cite{tonella2013interactive,xuan2012solving,saliu2005software} &
		\cellcolor{myblue!20}YES &
		\cellcolor{myblue!20}NO &
		\cellcolor{myblue!20}NO &
		\cellcolor{myblue!20}NO &
		\cellcolor{myblue!20}NO &
		\cellcolor{myblue!20}YES &
		\cellcolor{myblue!20}NO
		
		\bigstrut\\
		\cline{2-9} & 
		
		\cellcolor{myblue!20}\cite{li2016value} &
		\cellcolor{myblue!20}NO &
		\cellcolor{myblue!20}NO &
		\cellcolor{myblue!20}NO &
		\cellcolor{myblue!20}NO &
		\cellcolor{myblue!20}NO &
		\cellcolor{myblue!20}YES &
		\cellcolor{myblue!20}NO
		
		\bigstrut\\
		\hline
		
		\cellcolor{myblue!10} Increase/Decrease\_Value\_Of (subsets of size 2) &
		\cellcolor{myblue!10}\cite{li_integrated_2010,sagrado_multi_objective_2013,Zhang_RIM_2013}&
		\cellcolor{myblue!10}YES &
		\cellcolor{myblue!10}NO &
		\cellcolor{myblue!10}YES &
		\cellcolor{myblue!10}YES &
		\cellcolor{myblue!10}NO &
		\cellcolor{myblue!10}YES &
		\cellcolor{myblue!10}YES
		
		\bigstrut\\
		\hline
		
		\cellcolor{myblue!10} Increase/Decrease\_Value\_Of (subsets of any size) &
		\cellcolor{myblue!10}\cite{van_den_akker_flexible_2005}&
		\cellcolor{myblue!10}YES &
		\cellcolor{myblue!10}YES &
		\cellcolor{myblue!10}NO &
		\cellcolor{myblue!10}NO &
		\cellcolor{myblue!10}NO &
		\cellcolor{myblue!10}YES &
		\cellcolor{myblue!10}YES
		\\\bottomrule[1.5pt]
		
	\end{tabular}%
}



==> table_lr2.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet2'
\begin{tabular}{|l|l|lllllll|}
\hline
\textbf{\cellcolor{header}\textcolor{white}{Employed Model}} &
  \textbf{\cellcolor{header}\textcolor{white}{Works}} &
  \textbf{\cellcolor{header}\textcolor{white}{P1}} &
  \textbf{\cellcolor{header}\textcolor{white}{P2}} &
  \textbf{\cellcolor{header}\textcolor{white}{P3}} &
  \textbf{\cellcolor{header}\textcolor{white}{P4}} &
  \textbf{\cellcolor{header}\textcolor{white}{P5}} &
  \textbf{\cellcolor{header}\textcolor{white}{P6}} &
  \textbf{\cellcolor{header}\textcolor{white}{P7}}
  \bigstrut\\
\hline
BKP &
   &
   &
   &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  
  \bigstrut\\
\hline
\multirow{4}[8]{*}{BKP-PC} &
   &
   &
   &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  
  \bigstrut\\
\cline{2-9} &
   &
   &
   &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  
  \bigstrut\\
\cline{2-9} &
   &
   &
   &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  
  \bigstrut\\
\cline{2-9} &
   &
   &
   &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  
  \bigstrut\\
\hline
\multicolumn{1}{|l|}{\multirow{2}[4]{*}{Increase/Decrease\_Value\_Of}} &
   &
   &
   &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  
  \bigstrut\\
\cline{2-9}\multicolumn{1}{|l|}{} &
   &
   &
   &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  
  \bigstrut\\
\hline
\end{tabular}%

==> table_lr3.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet2'
\LARGE
%\rowcolors{1}{}{lightmyblue}
\resizebox {1\textwidth }{!}{% Table generated by Excel2LaTeX from sheet 'Sheet2'
	\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
		\toprule[1.5 pt]
		\textbf{\cellcolor{header}\textcolor{white}{Employed Model}} &
		\textbf{\cellcolor{header}\textcolor{white}{Works}} &
		\textbf{\cellcolor{header}\textcolor{white}{P1}} &
		\textbf{\cellcolor{header}\textcolor{white}{P2}} &
		\textbf{\cellcolor{header}\textcolor{white}{P3}} &
		\textbf{\cellcolor{header}\textcolor{white}{P4}} &
		\textbf{\cellcolor{header}\textcolor{white}{P5}} &
		\textbf{\cellcolor{header}\textcolor{white}{P6}} &
		\textbf{\cellcolor{header}\textcolor{white}{P7}} 
		%\textbf{\cellcolor{header}\textcolor{white}{P8}} 

		\bigstrut\\
		\hline
		BKP &
		\begin{tabular}[t]{@{}c@{}} \cite{karlsson_optimizing_1997,jung_optimizing_1998,zhang_multi_objective_2007,baker_search_2006,finkelstein2009search,zhang2011comparing,del2010ant,kumari2012software} \phantom{sssssssssssss} \end{tabular} &
		NO &
		NO &
		NO &
		NO &
		NO &
		NO &
		NO
		\bigstrut\\
		\hline
		\multirow{4}[9]{*}{BKP-PC} &
		\begin{tabular}[t]{@{}c@{}} \cite{veerapen2015integer,brasil_multiobjective_2012,sagrado_multi_objective_2013,bagnall_next_2001,greer_software_2004,boschetti_lagrangian_2014,ruhe_quantitative_2003,van2011quantitative,zhang2010search,tonella2010using,freitas2011software}\\ \cite{colares_new_2009,saliu2007bi,saliu2005supporting,jiang2010hybrid,van2005determination,ngo2009optimized,chen2013ant,del2011requirements,araujo2016architecture,colares2009new,pitangueira2016risk}\end{tabular} &
		NO  &
		NO  &
		NO  &
		NO  &
		YES &
		NO  &
		NO  
		\bigstrut\\
		%\cdashline{2-9}
		\cline{2-10} &
		\cite{van2008software,ngo_wicked_2008} &
		YES &
		YES &
		YES &
		NO  &
		YES &
		NO  &
		NO   
		\bigstrut\\
		\cline{2-10} &
		\cite{tonella2013interactive,xuan2012solving,saliu2005software} &
		YES &
		NO  &
		NO  &
		NO  &
		YES &
		NO  &
		NO 
		\bigstrut\\
		\hline
		\multicolumn{1}{|l|}{\multirow{2}[4]{*}{Increase-Decrease}} &
		\cite{li_integrated_2010,sagrado_multi_objective_2013,Zhang_RIM_2013} (subsets of size 2) &
		YES &
		NO  &
		YES &
		NO  &
		YES &
		NO  &
		YES 
		\bigstrut\\
		\cline{2-10}\multicolumn{1}{|l|}{} &
		\cite{van_den_akker_flexible_2005} (subsets of any size) &
		YES &
		YES &
		NO  &
		NO  &
		YES &
		NO  &
		YES 
		\bigstrut\\
		\hline
	\end{tabular}%
}


==> table_lr_new.tex <==
	\begin{tabular}{lllllll}
		&                                                                                         &                                                                                                               &                                                                                                                                                                                                                                                                         &                                                                                                     &                                                               &  \\ \cline{2-6}
		\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\textbf{Categories}}                                                & \multicolumn{1}{l|}{\textbf{BKP Models}}                                                                      & \multicolumn{1}{l|}{\textbf{BKP-PC Models}}                                                                                                                                                                                                                             & \multicolumn{2}{l|}{\textbf{Increase/Decrease-Value-of Models}}                                                                                                     &  \\ \cline{2-6}
		\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{Works from the Literature}                                          & \multicolumn{1}{l|}{\cite\{karlsson\_optimizing\_1997,jung\_optimizing\_1998,zhang\_multi\_objective\_2007\}} & \multicolumn{1}{l|}{\cite\{brasil\_multiobjective\_2012,li\_integrated\_2010,sagrado\_multi\_objective\_2013,boschetti\_lagrangian\_2014,brasil\_multiobjective\_2012,brasil\_multiobjective\_2012,bagnall\_next\_2001,Greer\_evolutionary\_2004,baker\_search\_2006\}} & \multicolumn{1}{l|}{\cite\{li\_integrated\_2010,sagrado\_multi\_objective\_2013,Zhang\_RIM\_2013\}} & \multicolumn{1}{l|}{\cite\{van\_den\_akker\_flexible\_2005\}} &  \\ \cline{2-6}
		\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}considers explicit value dependencies}      & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}NO}                                                               & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}YES}                                                                                                                                                                                                                        & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}YES}                                                    & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}YES}              &  \\ \cline{2-6}
		\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{considers implicit value dependencies}                              & \multicolumn{1}{l|}{NO}                                                                                       & \multicolumn{1}{l|}{YES}                                                                                                                                                                                                                                                & \multicolumn{1}{l|}{NO}                                                                             & \multicolumn{1}{l|}{NO}                                       &  \\ \cline{2-6}
		\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{considers qualities (positivity/negativity) of  value dependencies} & \multicolumn{1}{l|}{NO}                                                                                       & \multicolumn{1}{l|}{YES}                                                                                                                                                                                                                                                & \multicolumn{1}{l|}{YES}                                                                            & \multicolumn{1}{l|}{NO}                                       &  \\ \cline{2-6}
		\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{considers strengths of value dependencies}                          & \multicolumn{1}{l|}{NO}                                                                                       & \multicolumn{1}{l|}{NO}                                                                                                                                                                                                                                                 & \multicolumn{1}{l|}{NO}                                                                             & \multicolumn{1}{l|}{NO}                                       &  \\ \cline{2-6}
		\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{considers simultaneous positive and negative value dependencies}    & \multicolumn{1}{l|}{NO}                                                                                       & \multicolumn{1}{l|}{YES}                                                                                                                                                                                                                                                & \multicolumn{1}{l|}{NO}                                                                             & \multicolumn{1}{l|}{NO}                                       &  \\ \cline{2-6}
		\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{is prone to SDP}                                                    & \multicolumn{1}{l|}{NO}                                                                                       & \multicolumn{1}{l|}{YES}                                                                                                                                                                                                                                                & \multicolumn{1}{l|}{NO}                                                                             & \multicolumn{1}{l|}{NO}                                       &  \\ \cline{2-6}
		&                                                                                         &                                                                                                               &                                                                                                                                                                                                                                                                         &                                                                                                     &                                                               &  \\
		&                                                                                         &                                                                                                               &                                                                                                                                                                                                                                                                         &                                                                                                     &                                                               &  \\
		&                                                                                         &                                                                                                               &                                                                                                                                                                                                                                                                         &                                                                                                     &                                                               &  \\
		&                                                                                         &                                                                                                               &                                                                                                                                                                                                                                                                         &                                                                                                     &                                                               &  \\
		&                                                                                         &                                                                                                               &                                                                                                                                                                                                                                                                         &                                                                                                     &                                                               &  \\
		&                                                                                         &                                                                                                               &                                                                                                                                                                                                                                                                         &                                                                                                     &                                                               & 
	\end{tabular}


==> table_lr_old.tex <==
\rowcolors{1}{}{lightgray}
\LARGE\resizebox {1\textwidth }{!}{% Table generated by Excel2LaTeX from sheet 'Sheet1'
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{tabular}{l|l|l|l|l}
	\hline
	\multicolumn{1}{l|}{\multirow{2}[4]{*}{\textbf{Selection Model}}} &
	\multicolumn{1}{l|}{\multirow{2}[4]{*}{\textbf{BKP}}} &
	\multicolumn{1}{l|}{\multirow{2}[4]{*}{\textbf{BKP-PC}}} &
	\multicolumn{2}{c}{\textbf{Increase/Decrease-Value-of}}
	\bigstrut\\
	\cline{4-5}\multicolumn{1}{c|}{} &
	\multicolumn{1}{l|}{} &
	\multicolumn{1}{l|}{} &
	\multicolumn{1}{l|}{Subsets of Size 2 Only} &
	\multicolumn{1}{l}{Subsets of Any Size}
	\bigstrut\\
	\hline
	\multicolumn{1}{l|}{Sample works from the  literature} &
	\cite{karlsson_optimizing_1997,jung_optimizing_1998,zhang_multi_objective_2007}  &
	\cite{brasil_multiobjective_2012,li_integrated_2010,sagrado_multi_objective_2013,Greer_evolutionary_2004,boschetti_lagrangian_2014,bagnall_next_2001,baker_search_2006} &
	\cite{li_integrated_2010,sagrado_multi_objective_2013,Zhang_RIM_2013} &
	\cite{van_den_akker_flexible_2005}
	\bigstrut\\
	\hline
	Considers explicit value dependencies &
	NO &
	YES &
	YES &
	YES
	\bigstrut[t]\\
	Considers implicit value dependencies &
	NO &
	YES &
	NO &
	NO
	\\
	Considers qualities (positivity/negativity) of  value dependencies &
	NO &
	YES &
	YES &
	NO
	\\
	Considers strengths of value dependencies &
	NO &
	NO &
	NO &
	NO
	\\
	Considers simultaneous positive and negative value dependencies  &
	NO &
	YES &
	NO &
	NO
	\\
	Is prone to SDP &
	NO &
	YES &
	NO &
	NO
	\bigstrut[b]\\
	\hline
\end{tabular}
}




==> table_precede.tex <==
\huge\resizebox {1\textwidth }{!}{
\begin{tabular}{lllllllllllllllllllllllllllll}
\toprule[1.5pt]
\textbf{\cellcolor{black}\textcolor{white}{}}& \textbf{\cellcolor{black}\textcolor{white}{$f_{1}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{2}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{3}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{4}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{5}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{6}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{7}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{8}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{9}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{10}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{11}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{12}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{13}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{14}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{15}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{16}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{17}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{18}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{19}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{20}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{21}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{22}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{23}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{24}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{25}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{26}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{27}$}}
\\\midrule \addlinespace[0.4ex]
\textbf{\cellcolor{black}\textcolor{white}{$f_{1}$}}& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{2}$}}& \cellcolor{gray!30}$+1.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{3}$}}& \cellcolor{gray!30}$+1.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{4}$}}& $\pm0.00$& \cellcolor{gray!30}$+1.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{5}$}}& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{6}$}}& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{7}$}}& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{8}$}}& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& \cellcolor{gray!30}$+1.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{9}$}}& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& \cellcolor{gray!30}$+1.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{10}$}}& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{11}$}}& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{12}$}}& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{13}$}}& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& \cellcolor{gray!30}$+1.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{14}$}}& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{15}$}}& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{16}$}}& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{17}$}}& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{18}$}}& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& \cellcolor{gray!30}$+1.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{19}$}}& $\pm0.00$& \cellcolor{gray!30}$+1.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& \cellcolor{gray!30}$+1.00$& $\pm0.00$& $\pm0.00$& \cellcolor{gray!30}$+1.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{20}$}}& $\pm0.00$& \cellcolor{gray!30}$+1.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& \cellcolor{gray!30}$+1.00$& $\pm0.00$& $\pm0.00$& \cellcolor{gray!30}$+1.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{21}$}}& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{22}$}}& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{23}$}}& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{24}$}}& \cellcolor{gray!30}$+1.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{25}$}}& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{26}$}}& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& \cellcolor{gray!30}$+1.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{27}$}}& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\addlinespace[0.4ex]\toprule[1.5pt]
\end{tabular}}

==> table_rho.tex <==
\huge\resizebox {1\textwidth }{!}{
\begin{tabular}{lllllllllllllllllllllllllllll}
\toprule[1.5pt]
\textbf{\cellcolor{black}\textcolor{white}{}}& \textbf{\cellcolor{black}\textcolor{white}{$f_{1}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{2}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{3}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{4}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{5}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{6}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{7}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{8}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{9}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{10}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{11}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{12}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{13}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{14}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{15}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{16}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{17}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{18}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{19}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{20}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{21}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{22}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{23}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{24}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{25}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{26}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{27}$}}
\\\midrule \addlinespace[0.4ex]
\textbf{\cellcolor{black}\textcolor{white}{$f_{1}$}}& $\pm0.00$& $+0.14$& $+0.09$& $+0.03$& $+0.14$& $+0.01$& $+0.01$& $+0.16$& $+0.03$& $+0.03$& $-0.02$& $+0.11$& $+0.03$& $+0.11$& $+0.15$& $+0.09$& $+0.01$& $-0.04$& $-0.04$& $-0.04$& $-0.02$& $+0.06$& $+0.14$& $+0.14$& $-0.14$& $-0.18$& $-0.01$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{2}$}}& $+0.16$& $\pm0.00$& $+0.20$& $+0.47$& $+1.00$& $+0.07$& $+0.02$& $+0.25$& $+0.47$& $+0.47$& $+0.25$& $+0.07$& $+0.47$& $+0.22$& $+0.24$& $+0.43$& $+0.22$& $+0.24$& $+0.12$& $+0.17$& $+0.18$& $+0.19$& $+1.00$& $+1.00$& $+0.18$& $+0.00$& $+0.15$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{3}$}}& $+0.18$& $+0.37$& $\pm0.00$& $+0.40$& $+0.37$& $-0.00$& $+0.15$& $+0.47$& $+0.40$& $+0.40$& $+0.33$& $-0.15$& $+0.40$& $+0.68$& $+0.50$& $+0.35$& $-0.07$& $+0.07$& $+0.01$& $+0.09$& $+0.48$& $+0.33$& $+0.37$& $+0.37$& $+0.00$& $-0.06$& $+0.02$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{4}$}}& $+0.05$& $+0.72$& $+0.32$& $\pm0.00$& $+0.72$& $+0.30$& $-0.02$& $+0.42$& $+1.00$& $+1.00$& $+0.39$& $+0.03$& $+1.00$& $+0.33$& $+0.39$& $+0.40$& $+0.12$& $+0.37$& $-0.00$& $+0.25$& $+0.27$& $+0.30$& $+0.72$& $+0.72$& $+0.27$& $-0.11$& $+0.24$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{5}$}}& $+0.16$& $+1.00$& $+0.20$& $+0.47$& $\pm0.00$& $+0.07$& $+0.02$& $+0.25$& $+0.47$& $+0.47$& $+0.25$& $+0.07$& $+0.47$& $+0.22$& $+0.24$& $+0.43$& $+0.22$& $+0.24$& $+0.12$& $+0.17$& $+0.18$& $+0.19$& $+1.00$& $+1.00$& $+0.18$& $+0.00$& $+0.15$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{6}$}}& $+0.02$& $+0.11$& $-0.00$& $+0.33$& $+0.11$& $\pm0.00$& $-0.05$& $+0.13$& $+0.33$& $+0.33$& $+0.14$& $+0.32$& $+0.33$& $+0.05$& $+0.09$& $-0.03$& $-0.19$& $+0.08$& $-0.37$& $+0.27$& $-0.25$& $-0.03$& $+0.11$& $+0.11$& $+0.04$& $-0.49$& $+0.30$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{7}$}}& $+0.01$& $+0.04$& $+0.11$& $-0.02$& $+0.04$& $-0.04$& $\pm0.00$& $-0.11$& $-0.02$& $-0.02$& $+0.21$& $-0.14$& $-0.02$& $+0.12$& $-0.14$& $-0.04$& $-0.10$& $-0.16$& $-0.09$& $+0.17$& $-0.03$& $-0.23$& $+0.04$& $+0.04$& $-0.04$& $+0.02$& $+0.16$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{8}$}}& $+0.33$& $+0.46$& $+0.47$& $+0.51$& $+0.46$& $+0.14$& $-0.15$& $\pm0.00$& $+0.51$& $+0.51$& $+0.24$& $-0.07$& $+0.51$& $+0.54$& $+0.70$& $+0.25$& $+0.01$& $+0.21$& $-0.11$& $-0.09$& $+0.36$& $+0.43$& $+0.46$& $+0.46$& $-0.05$& $-0.24$& $-0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{9}$}}& $+0.05$& $+0.72$& $+0.32$& $+1.00$& $+0.72$& $+0.30$& $-0.02$& $+0.42$& $\pm0.00$& $+1.00$& $+0.39$& $+0.03$& $+1.00$& $+0.33$& $+0.39$& $+0.40$& $+0.12$& $+0.37$& $-0.00$& $+0.25$& $+0.27$& $+0.30$& $+0.72$& $+0.72$& $+0.27$& $-0.11$& $+0.24$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{10}$}}& $+0.05$& $+0.72$& $+0.32$& $+1.00$& $+0.72$& $+0.30$& $-0.02$& $+0.42$& $+1.00$& $\pm0.00$& $+0.39$& $+0.03$& $+1.00$& $+0.33$& $+0.39$& $+0.40$& $+0.12$& $+0.37$& $-0.00$& $+0.25$& $+0.27$& $+0.30$& $+0.72$& $+0.72$& $+0.27$& $-0.11$& $+0.24$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{11}$}}& $-0.04$& $+0.49$& $+0.34$& $+0.49$& $+0.49$& $+0.16$& $+0.29$& $+0.25$& $+0.49$& $+0.49$& $\pm0.00$& $-0.04$& $+0.49$& $+0.42$& $+0.20$& $+0.26$& $+0.10$& $+0.28$& $+0.00$& $+0.42$& $+0.36$& $-0.02$& $+0.49$& $+0.49$& $+0.24$& $-0.06$& $+0.24$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{12}$}}& $+0.15$& $+0.08$& $-0.10$& $+0.03$& $+0.08$& $+0.22$& $-0.11$& $-0.04$& $+0.03$& $+0.03$& $-0.02$& $\pm0.00$& $+0.03$& $-0.10$& $-0.06$& $+0.02$& $-0.02$& $-0.06$& $-0.04$& $+0.17$& $-0.26$& $-0.11$& $+0.08$& $+0.08$& $+0.01$& $-0.20$& $+0.17$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{13}$}}& $+0.05$& $+0.72$& $+0.32$& $+1.00$& $+0.72$& $+0.30$& $-0.02$& $+0.42$& $+1.00$& $+1.00$& $+0.39$& $+0.03$& $\pm0.00$& $+0.33$& $+0.39$& $+0.40$& $+0.12$& $+0.37$& $-0.00$& $+0.25$& $+0.27$& $+0.30$& $+0.72$& $+0.72$& $+0.27$& $-0.11$& $+0.24$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{14}$}}& $+0.25$& $+0.43$& $+0.71$& $+0.43$& $+0.43$& $+0.06$& $+0.17$& $+0.57$& $+0.43$& $+0.43$& $+0.42$& $-0.16$& $+0.43$& $\pm0.00$& $+0.59$& $+0.37$& $-0.00$& $+0.14$& $-0.11$& $+0.10$& $+0.46$& $+0.27$& $+0.43$& $+0.43$& $-0.06$& $-0.18$& $-0.03$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{15}$}}& $+0.32$& $+0.47$& $+0.52$& $+0.50$& $+0.47$& $+0.10$& $-0.20$& $+0.73$& $+0.50$& $+0.50$& $+0.20$& $-0.09$& $+0.50$& $+0.58$& $\pm0.00$& $+0.48$& $+0.10$& $+0.30$& $-0.01$& $-0.04$& $+0.42$& $+0.51$& $+0.47$& $+0.47$& $+0.02$& $-0.17$& $-0.13$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{16}$}}& $+0.14$& $+0.59$& $+0.25$& $+0.36$& $+0.59$& $-0.02$& $-0.04$& $+0.18$& $+0.36$& $+0.36$& $+0.18$& $+0.02$& $+0.36$& $+0.26$& $+0.33$& $\pm0.00$& $+0.31$& $+0.30$& $+0.25$& $+0.20$& $+0.25$& $+0.24$& $+0.59$& $+0.59$& $+0.23$& $+0.08$& $-0.01$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{17}$}}& $+0.02$& $+0.41$& $-0.07$& $+0.15$& $+0.41$& $-0.22$& $-0.13$& $+0.01$& $+0.15$& $+0.15$& $+0.10$& $-0.03$& $+0.15$& $-0.00$& $+0.10$& $+0.44$& $\pm0.00$& $+0.52$& $+0.49$& $+0.12$& $+0.33$& $+0.24$& $+0.41$& $+0.41$& $+0.42$& $+0.32$& $-0.01$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{18}$}}& $-0.10$& $+0.48$& $+0.08$& $+0.47$& $+0.48$& $+0.09$& $-0.23$& $+0.22$& $+0.47$& $+0.47$& $+0.28$& $-0.09$& $+0.47$& $+0.14$& $+0.30$& $+0.44$& $+0.54$& $\pm0.00$& $+0.29$& $+0.22$& $+0.46$& $+0.39$& $+0.48$& $+0.48$& $+0.57$& $+0.16$& $+0.07$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{19}$}}& $-0.08$& $+0.21$& $+0.01$& $-0.00$& $+0.21$& $-0.39$& $-0.11$& $-0.11$& $-0.00$& $-0.00$& $+0.00$& $-0.06$& $-0.00$& $-0.10$& $-0.01$& $+0.33$& $+0.47$& $+0.26$& $\pm0.00$& $+0.03$& $+0.31$& $+0.17$& $+0.21$& $+0.21$& $+0.35$& $+0.49$& $-0.11$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{20}$}}& $-0.07$& $+0.26$& $+0.08$& $+0.26$& $+0.26$& $+0.25$& $+0.19$& $-0.07$& $+0.26$& $+0.26$& $+0.33$& $+0.22$& $+0.26$& $+0.08$& $-0.03$& $+0.23$& $+0.10$& $+0.17$& $+0.03$& $\pm0.00$& $+0.01$& $-0.10$& $+0.26$& $+0.26$& $+0.36$& $-0.05$& $+0.42$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{21}$}}& $-0.03$& $+0.23$& $+0.33$& $+0.22$& $+0.23$& $-0.19$& $-0.03$& $+0.25$& $+0.22$& $+0.22$& $+0.24$& $-0.28$& $+0.22$& $+0.30$& $+0.28$& $+0.24$& $+0.23$& $+0.30$& $+0.22$& $+0.01$& $\pm0.00$& $+0.33$& $+0.23$& $+0.23$& $+0.23$& $+0.22$& $-0.09$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{22}$}}& $+0.12$& $+0.34$& $+0.32$& $+0.35$& $+0.34$& $-0.03$& $-0.29$& $+0.42$& $+0.35$& $+0.35$& $-0.01$& $-0.16$& $+0.35$& $+0.25$& $+0.48$& $+0.33$& $+0.23$& $+0.36$& $+0.17$& $-0.12$& $+0.47$& $\pm0.00$& $+0.34$& $+0.34$& $+0.24$& $+0.11$& $-0.01$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{23}$}}& $+0.16$& $+1.00$& $+0.20$& $+0.47$& $+1.00$& $+0.07$& $+0.02$& $+0.25$& $+0.47$& $+0.47$& $+0.25$& $+0.07$& $+0.47$& $+0.22$& $+0.24$& $+0.43$& $+0.22$& $+0.24$& $+0.12$& $+0.17$& $+0.18$& $+0.19$& $\pm0.00$& $+1.00$& $+0.18$& $+0.00$& $+0.15$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{24}$}}& $+0.16$& $+1.00$& $+0.20$& $+0.47$& $+1.00$& $+0.07$& $+0.02$& $+0.25$& $+0.47$& $+0.47$& $+0.25$& $+0.07$& $+0.47$& $+0.22$& $+0.24$& $+0.43$& $+0.22$& $+0.24$& $+0.12$& $+0.17$& $+0.18$& $+0.19$& $+1.00$& $\pm0.00$& $+0.18$& $+0.00$& $+0.15$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{25}$}}& $-0.25$& $+0.29$& $+0.00$& $+0.28$& $+0.29$& $+0.04$& $-0.04$& $-0.04$& $+0.28$& $+0.28$& $+0.20$& $+0.01$& $+0.28$& $-0.05$& $+0.02$& $+0.27$& $+0.36$& $+0.47$& $+0.32$& $+0.38$& $+0.29$& $+0.21$& $+0.29$& $+0.29$& $\pm0.00$& $+0.30$& $+0.27$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{26}$}}& $-0.37$& $+0.01$& $-0.06$& $-0.13$& $+0.01$& $-0.53$& $+0.02$& $-0.24$& $-0.13$& $-0.13$& $-0.06$& $-0.30$& $-0.13$& $-0.17$& $-0.16$& $+0.11$& $+0.31$& $+0.15$& $+0.50$& $-0.06$& $+0.31$& $+0.11$& $+0.01$& $+0.01$& $+0.34$& $\pm0.00$& $-0.11$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{27}$}}& $-0.01$& $+0.25$& $+0.01$& $+0.27$& $+0.25$& $+0.30$& $+0.19$& $-0.00$& $+0.27$& $+0.27$& $+0.20$& $+0.24$& $+0.27$& $-0.02$& $-0.11$& $-0.01$& $-0.01$& $+0.06$& $-0.10$& $+0.46$& $-0.12$& $-0.01$& $+0.25$& $+0.25$& $+0.28$& $-0.10$& $\pm0.00$\\
\addlinespace[0.4ex]\toprule[1.5pt]
\end{tabular}}

==> table_sigma.tex <==
\resizebox {0.5\textwidth }{!}{
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{tabular}{lllll}
	\boldmath{}\textbf{$\sigma_{I,j}$}\unboldmath{} &
	\boldmath{}\textbf{$r_1$}\unboldmath{} &
	\boldmath{}\textbf{$r_2$}\unboldmath{} &
	\boldmath{}\textbf{$r_3$}\unboldmath{} &
	\boldmath{}\textbf{$r_4$}\unboldmath{}
	\\
	\boldmath{}\textbf{$r_1$}\unboldmath{} &
	&
	&
	&
	
	\\
	\boldmath{}\textbf{$r_2$}\unboldmath{} &
	&
	&
	&
	
	\\
	\boldmath{}\textbf{$r_3$}\unboldmath{} &
	&
	&
	&
	
	\\
	\boldmath{}\textbf{$r_4$}\unboldmath{} &
	&
	&
	&
	
	\\
\end{tabular}%
}


==> table_sim_design.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\resizebox {1\textwidth }{!}{
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{tabular}{|l|l|l|l|l|}
	\cmidrule[1pt]{2-5}
	\multicolumn{1}{l|}{} 
	&
	\cellcolor{gray!30}\textbf{VDL=[0,1]} &
	\cellcolor{gray!30}\textbf{NVDL=[0,1]} &
	\cellcolor{gray!30}\textbf{PDL=[0,1]} & 
	\cellcolor{gray!30}\textbf{NPDL=[0,1]} 
	\bigstrut\\
	\hline
	\cellcolor{gray!30}$\%$\textbf{Budget=[0,100]} &
	NVDL=0.0,PDL=0.02,NPDL=0.0  &
	VDL=0.15,PDL=0.02,NPDL=0.0  &
	VDL=0.15,NVDL=0.0,NPDL=0.0 & 
	VDL=0.15,NVDL=0.0,PDL=0.02
	\bigstrut\\
	\hline
	\cellcolor{gray!30}\textbf{VDL=[0,1]} &
	&
	$\%$Budget=95, PDL=0.02, NPDL=0.0 &
	$\%$Budget=95,NVDL=0.0, NPDL=0.0 &
	$\%$Budget=95,NVDL=0.0, PDL=0.02
	\bigstrut\\
	\hline
	\cellcolor{gray!30}\textbf{NVDL=[0,1]} &
	&
	&
	$\%$Budget=95,VDL=0.15, NPDL=0.0 &
	$\%$Budget=95,VDL=0.15, PDL=0.02
	\bigstrut\\
	\hline
	\cellcolor{gray!30}\textbf{PDL=[0,1]} &
	&
	&
	& 
	$\%$Budget=95, VDL=0.15, NVDL=0.0 
	\bigstrut\\
	\bottomrule
\end{tabular}%
}

==> table_sim_design_all.tex <==
% Table generated by Excel2LaTeX from sheet 'table_sim_design_all'
\resizebox {0.7\textwidth }{!}{
	\begin{tabular}{clllll}
	\toprule[1.5pt]
	\rowcolor{gray!30}
	\textbf{\cellcolor{black}\textcolor{white}{Simulation}} &
	\textbf{\cellcolor{black}\textcolor{white}{$\%$Budget}} &
	\textbf{\cellcolor{black}\textcolor{white}{VDL}} &
	\textbf{\cellcolor{black}\textcolor{white}{NVDL}} &
    \textbf{\cellcolor{black}\textcolor{white}{PDL}} &
	\textbf{\cellcolor{black}\textcolor{white}{NPDL}} 
	\bigstrut\\
	\rowcolor{gray!25}
	%\hline
	I &
	[0,100] &
	[0,1] &
	0.00&
	0.02 &
	0.00
	\bigstrut\\
	%\hline
	II &
	[0,100] &
	0.15 &
	[0,1] &
	0.02 &
	0.00
	\bigstrut\\
	\rowcolor{gray!25}
	%\hline
	III &
	[0,100] &
	0.15 &
	0.00&
	[0,1] &
	0.00
	\bigstrut\\
	%\hline
	IV &
	[0,100] &
	0.15 &
	0.00&
	0.02 &
	[0,1]
	\bigstrut\\
	\rowcolor{gray!25}
	%\hline
	V &
	95 &
	[0,1] &
	[0,1] &
	0.02 &
	0.00
	\bigstrut\\
	%\hline
	VI &
	95 &
	0.15 &
	0.00&
	[0,1] &
	[0,1]
	\bigstrut\\
	\bottomrule[1.5pt]
\end{tabular}
}


==> table_sim_design_all_previous.tex <==
% Table generated by Excel2LaTeX from sheet 'table_sim_design_all'
\resizebox {0.7\textwidth }{!}{
	\begin{tabular}{clllll}
	\toprule[1.5pt]
	\rowcolor{gray!30}
	\textbf{\cellcolor{black}\textcolor{white}{Simulation}} &
	\textbf{\cellcolor{black}\textcolor{white}{$\%$Budget}} &
	\textbf{\cellcolor{black}\textcolor{white}{VDL}} &
	\textbf{\cellcolor{black}\textcolor{white}{NVDL}} &
    \textbf{\cellcolor{black}\textcolor{white}{PDL}} &
	\textbf{\cellcolor{black}\textcolor{white}{NPDL}} 
	\bigstrut\\
	\rowcolor{gray!25}
	%\hline
	I &
	[0,1] &
	[0,1] &
	0.00&
	0.02 &
	0.00
	\bigstrut\\
	%\hline
	II &
	[0,1] &
	0.15 &
	[0,1] &
	0.02 &
	0.00
	\bigstrut\\
	\rowcolor{gray!25}
	%\hline
	III &
	[0,1] &
	0.15 &
	0.00&
	[0,1] &
	0.00
	\bigstrut\\
	%\hline
	IV &
	[0,1] &
	0.15 &
	0.00&
	0.02 &
	[0,1]
	\bigstrut\\
	\rowcolor{gray!25}
	%\hline
	V &
	0.95 &
	[0,1] &
	[0,1] &
	0.02 &
	0.00
	\bigstrut\\
	%\hline
	VI &
	0.95 &
	[0,1] &
	0.00&
	[0,1] &
	0.00
	\bigstrut\\
	\rowcolor{gray!25}
	%\hline
	VII &
	0.95 &
	[0,1] &
	0.00&
	0.02 &
	[0,1]
	\bigstrut\\
	%\hline
	VIII &
	0.95 &
	0.15 &
	[0,1] &
	[0,1] &
	0.00
	\bigstrut\\
	\rowcolor{gray!25}
	%\hline
	IX &
	0.95 &
	0.15 &
	[0,1] &
	0.02 &
	[0,1]
	\bigstrut\\
	\rowcolor{gray!25}
	%\hline
	X &
	0.95 &
	0.15 &
	0.00&
	[0,1] &
	[0,1]
	\bigstrut\\
	\bottomrule[1.5pt]
\end{tabular}
}


==> table_sim_scalability_design_previous.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\resizebox {0.75\textwidth }{!}{
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{tabular}{lllllll}
	\toprule[1.5pt]
	\rowcolor{gray!30}
	\textbf{\cellcolor{black}\textcolor{white}{Simulation}} &
	\textbf{\cellcolor{black}\textcolor{white}{Size}} &
	\textbf{\cellcolor{black}\textcolor{white}{$\%$Budget}} &
	\textbf{\cellcolor{black}\textcolor{white}{VDL}} &
	\textbf{\cellcolor{black}\textcolor{white}{NVDL}} &
	\textbf{\cellcolor{black}\textcolor{white}{PDL}} &
	\textbf{\cellcolor{black}\textcolor{white}{NPDL}}
	\bigstrut\\
	\hline
	XI &
	[0,2000] &
	50 &
	0.15 &
	0.00 &
	0.02 &
	0.00
	\bigstrut\\ \rowcolor{gray!25}
	XII &
	200 &
	[0,100] &
	0.15 &
	0.00 &
	0.02 &
	0.00
    \bigstrut\\
	XIII &
	[0,1000] &
	[0,100] &
	0.15 &
	0.00 &
	0.02 &
	0.00
	\bigstrut\\	\rowcolor{gray!25}
	XIV &
	200 &
	50 &
	0.15 &
	0.00 &
	[0,0.007] &
	0.00
	\bigstrut\\	
	XV &
	200 &
	50 &
	0.15 &
	0 &
    [0.007,1] &
	0.00
	\bigstrut\\ \rowcolor{gray!25}
	XVI &
	200 &
	50 &
	[0,1] &
	[0,1] &
	0.02 &
	0.00
	\bigstrut\\
	XVII &
	200 &
	50 &
	0.15 &
	0.00 &
	[0,1] &
	0.00
	\bigstrut\\ \rowcolor{gray!25}
	XVIII &
	200 &
	50 &
	0.15 &
	0.00 &
	0.02 &
	[0,1]
	\bigstrut\\
	XIX &
	200 &
	50 &
	0.15 &
	0.00 &
	[0,1] &
	[0,1]
	\bigstrut\\ 
	\bottomrule[1.5pt]
\end{tabular}
}

==> table_types_intrinsic.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\LARGE
%\rowcolors{1}{}{myblue!20}
\resizebox {1\textwidth }{!}{% Table generated by Excel2LaTeX from sheet 'Sheet1'
	\begin{tabular}{|l|l|l|}
		\toprule[1.5 pt]
		\textbf{\cellcolor{header}\textcolor{white}{Dependency Type}} &
		\textbf{\cellcolor{header}\textcolor{white}{Description}} &
		\textbf{\cellcolor{header}\textcolor{white}{Example}}
		\bigstrut\\
		\hline
		\begin{tabular}[c]{@{}l@{}}Constrain~\cite{zhang_investigating_2014,k_process_centered_1996}\end{tabular} &
	    \begin{tabular}[c]{@{}l@{}}\textit{ }\textbullet\textit{ }One requirement is a constraint of another requirement.\end{tabular}  &
		\begin{tabular}[c]{@{}l@{}}			
			\textit{ }\textbullet\textit{ } $r_1:$ system should respond to users in 3 seconds \\
			\textit{ }\textbullet\textit{ } $r_2:$ users search books using book title or ID \\
			\textit{ }\textbullet\textit{ } $r_1$ constrains $r_2$
		\end{tabular}
		\bigstrut\\ \hline
		
		\begin{tabular}[c]{@{}l@{}}Precede~\cite{zhang_investigating_2014}, Precondition~\cite{k_process_centered_1996}, Requires~\cite{dahlstedt2005requirements}\end{tabular} &
		\begin{tabular}[c]{@{}l@{}}\textit{ }\textbullet\textit{ } If function A precedes function B\end{tabular} &
		\begin{tabular}[c]{@{}l@{}}			
			\textit{ }\textbullet\textit{ } $r_1:$ a client initiates a valuation request and the system checks the quality of the request\\
			\textit{ }\textbullet\textit{ } $r_2:$ users search books using book title or ID\\
			\textit{ }\textbullet\textit{ } $r_1$ precedes $r_2$\\
		\end{tabular}
		\bigstrut\\ \hline
		
		\begin{tabular}[c]{@{}l@{}}Be\_similar\_to~\cite{zhang_investigating_2014}, Similar~\cite{k_process_centered_1996}, Similar\_to~\cite{dahlstedt2005requirements}\end{tabular} &
		\begin{tabular}[c]{@{}l@{}}
				\textit{ }\textbullet\textit{ } (a) If two requirements share similar data information.\\ 
				\textit{ }\textbullet\textit{ } (b) If two requirements complete similar tasks.
		\end{tabular} &
		\begin{tabular}[c]{@{}l@{}}
				\textit{ }\textbullet\textit{ } (a) Adding a new book record is similar to modifying an old book as they share the book record.\\
				\textit{ }\textbullet\textit{ } (b) A property valuation could be complemented through curbside or desktop valuation.
		\end{tabular}
		\bigstrut\\ \hline
		
		\begin{tabular}[c]{@{}l@{}}Conflicts~\cite{zhang_investigating_2014,k_process_centered_1996}, Conflicts\_with~\cite{dahlstedt2005requirements}\end{tabular} &
		\begin{tabular}[c]{@{}l@{}} \textit{ }\textbullet\textit{ }One requirement may negatively impact another one.\end{tabular} &
		\textit{ }\textbullet\textit{ } Security may conflicts with performance.
		\bigstrut\\ \hline
		
		\begin{tabular}[c]{@{}l@{}}Be\_exception\_of~\cite{zhang_investigating_2014}\end{tabular} &
		\begin{tabular}[c]{@{}l@{}}\textit{ }\textbullet\textit{ }One requirement is an exceptional event of another one.\end{tabular} &
		\begin{tabular}[c]{@{}l@{}}
			\textit{ }\textbullet\textit{ } $r_1:$ A user inputs a null username and  system  reminds  him to correct it.\\
			\textit{ }\textbullet\textit{ } $r_2:$ A  user inputs his  username and  password  and  system checks validity of his information.\\
			\textit{ }\textbullet\textit{ } $r_1$ is an exception of $r_2$. 
		\end{tabular}
		\bigstrut\\ \hline
		
		\begin{tabular}[c]{@{}l@{}}Evolve\_into~\cite{zhang_investigating_2014}, Replaces~\cite{k_process_centered_1996}, Satisfies~\cite{k_process_centered_1996},\\ Based\_on~\cite{k_process_centered_1996}, Changes\_to~\cite{dahlstedt2005requirements}\end{tabular} &
		\begin{tabular}[c]{@{}l@{}} \textbullet\textit{ } Requirement $r_1$ is a new version of $r_2$. \end{tabular} &
		\begin{tabular}[c]{@{}l@{}}
			\textit{ }\textbullet\textit{ } $r_1:$ clients  use a desktop  PC  to upload  reports.\\
			\textit{ }\textbullet\textit{ } $r_2:$ clients use PDA to upload reports.\\
			\textit{ }\textbullet\textit{ } $r_1$ evolves into $r_2$. \\
		\end{tabular}
		\bigstrut\\ \hline
		
		\begin{tabular}[c]{@{}l@{}}Refines~\cite{zhang_investigating_2014,k_process_centered_1996}, Refines\_to~\cite{dahlstedt2005requirements}\end{tabular}&
		\begin{tabular}[c]{@{}l@{}} \textbullet\textit{ }One requirement is refined by more specific requirements.\end{tabular} &
		\begin{tabular}[c]{@{}l@{}}
			\textit{ }\textbullet\textit{ } $r_1:$ a valuer submit a valuation report.\\
			\textit{ }\textbullet\textit{ } $r_2:$ a valuer submits a report through web system.\\
			\textit{ }\textbullet\textit{ } $r_1$ is refined as $r_2$. 
		\end{tabular}
		\bigstrut\\
		\bottomrule[1.5pt]
	\end{tabular}
	}%


==> table_types_others.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
    \resizebox {1\textwidth }{!}{\begin{tabular}{|<{\centering}m{5cm}|<{\centering}m{10cm}|<{\centering}m{10cm}|<{\centering}m{5cm}|<{\centering}m{5cm}|}
\Xhline{4\arrayrulewidth}
\textbf{Dependency type} &
\textbf{Description} &
\textbf{Example} &
\textbf{Has Value (Dollars or Customer Satisfaction) Influences? }&
\textbf{Has Cost Influences?}
\bigstrut\\
\hline
Refined\_to 
& A higher-level requirement is refined by a number of more specific
requirements. 
& For a website, the requirement $r_1:$ \textit{authenticate users} can be refined to a more specific requirement $r_2:$ \textit{check user-name and password of users}.  
& YES~\cite{Robinson_RIM_2003,axel_reasoning_2004}. 
& YES~\cite{zhang_investigating_2014}

\bigstrut\\
\hline
Requires 
& Satisfaction of requirement $r_1$ to some extent \cite{dahlstedt_requirements_2005} depends on the satisfaction of requirement $r_2$. In case the dependency is strong $r_1$ can not be satisfied to any extent without $r_2$ in other cases, $r_1$ can still be partially satisfied without $r_2$ 
& Examples 1(Strong dependency): Sending an email requires a network connection, but not the opposite~\cite{carlshamre_industrial_2001} Examples 2(Week dependency):   
& YES~\cite{carlshamre_industrial_2001,carlshamre_release_2002,zhang_investigating_2014,dahlstedt_moulding_2003,dahlstedt_requirements_2005}. 
& YES~\cite{zhang_investigating_2014}

\bigstrut\\
\hline
Conflicts\_with
& Satisfaction of requirement $r_1$ strongly depends on the dissatisfaction of requirement $r_2$ to the extent that $r_1$ can not be satisfied to any extent when $r_2$ is even partially satisfied 
& If one requirement states that “All personnel should be able to search for information about both products and customers” and another states that “Only personnel with security status A should be able to search for customers classified as military related,” these two contradict each other, and cannot be simultaneously satisfied~\cite{dahlstedt_requirements_2005}.&
YES~\cite{carlshamre_industrial_2001,carlshamre_release_2002,zhang_investigating_2014,dahlstedt_moulding_2003,dahlstedt_requirements_2005}.
& YES~\cite{zhang_investigating_2014}

\bigstrut\\
\hline
AND 
& Is a bidirectional form of \texit{Requires} relation in which none of the AND-ed relations can be satisfied without the other one being fully satisfied. 
& a printer requires a driver to function, and the driver requires a printer to function~\cite{carlshamre_industrial_2001}. 
& YES, and discussed in the literature~\cite{carlshamre_industrial_2001,carlshamre_release_2002,zhang_investigating_2014,dahlstedt_moulding_2003,dahlstedt_requirements_2005}
& YES~\cite{zhang_investigating_2014}

\bigstrut\\
\hline
Increase/Decrease Value of 
& A requirement increases/decreases the value of another requirement without influencing its satisfaction. 
& Example 1: A detailed online manual may decrease the customer value of a printed manual~\cite{carlshamre_industrial_2001}. Example 2: The customer satisfaction of including a planning calendar into a mobile phone will probably increase if it is possible to synchronize this with planning calendars used on PCs 
& YES, and discussed in the literature~\cite{carlshamre_industrial_2001,carlshamre_release_2002,zhang_investigating_2014,dahlstedt_moulding_2003,dahlstedt_requirements_2005}.
& UNSPECIFIED

\bigstrut\\
\hline
Increase/Decrease Cost of 
& A requirement increases/decreases the cost of another requirement without influencing its satisfaction. 
& A requirement stating that ‘no response time should be longer than 1 second’ will typically increase the cost of implementing many other requirements~\cite{carlshamre_industrial_2001}. 
& NO 
& YES, and discussed in the literature~\cite{carlshamre_industrial_2001,carlshamre_release_2002,zhang_investigating_2014,dahlstedt_moulding_2003,dahlstedt_requirements_2005}.

\bigstrut\\
\Xhline{4\arrayrulewidth}
\end{tabular}}

==> table_types_robinson.tex <==
\resizebox {1\textwidth }{!}{\begin{tabular}{|l|l|}
\Xhline{4\arrayrulewidth}
\textbf{Dependency type} &
\textbf{Description} 

\bigstrut\\
\hline
Positive Influence(Interaction) 
& Increasing the satisfaction(value) of requirement $r_1$ will increase the satisfaction(value) of requirement $r_2$.

\bigstrut\\
\hline
Negative Influence(Interaction) 
& Increasing the satisfaction(value) of requirement $r_1$ will decreases the satisfaction(value) of requirement $r_2$. 

\bigstrut\\
\hline
Unspecified Influence(Interaction)
& Changing the satisfaction(value) of requirement $r_1$ has an unspecified influence on satisfaction(value) of requirement $r_2$.

\bigstrut\\
\hline
No Influence (Interaction) 
& Changing the satisfaction(value) of requirement $r_1$ has no influence on satisfaction(value) of requirement $r_2$. 

\bigstrut\\
\Xhline{4\arrayrulewidth}
\end{tabular}}

==> table_types_zhang.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet2'
\large\resizebox {1\textwidth }{!}{\begin{tabular}{|<{\centering}m{1.95cm}|<{\centering}m{4.8cm}|<{\centering}m{5.2cm}|<{\centering}m{8cm}|<{\centering}m{12cm}|}
\Xhline{4\arrayrulewidth}
\textbf{Category} &
\textbf{Types in Zhanng's model} &
\textbf{Corresponding types in other models} &
\textbf{Definition} &
\textbf{Example}

%--------------------------------------------------------
\bigstrut\\
\Xhline{4\arrayrulewidth}
intrinsic
& Constrain
& Constrain~\cite{k_process_centered_1996} 
& One requirement is a constraint of another requirement. This kind of dependency can represent crosscutting relationships among requirements.
& ‘system should respond to users in 3 seconds, constrains ‘book search function’ (user searches books using book title or ID).
%--------------------------------------------------------
\bigstrut\\
\cline{2-5} 
& Precede
& Precondition~\cite{k_process_centered_1996}, Requires~\cite{dahlstedt_requirements_2005}
& If function A precedes function B, A is a precondition of B.
& Given Requirement A:‘a client proposes the valuation request and system checks the quality of request’ and Requirement B:‘after the quality of request is checked, system allocates the valuation task to a valuer’, then A precedes B.
%--------------------------------------------------------
\bigstrut\\
\cline{2-5} 
& Be\_similar\_to
& Similar~\cite{k_process_centered_1996}, Similar\_to~\cite{dahlstedt_requirements_2005}
& a) If two requirements share similar data information, they are similar to each other. b) If two requirements complete similar tasks, they are similar to each other.
& a) Requirement ‘system administrator adds a new book re-cord’ is similar to ‘system administrator modiﬁes an old book record’. Book record in these two requirements is identical. b) After a client proposes a property valuation request, one valuer can choose from several options to evaluate the property,such as ‘desktop valuation’, ‘curbside valuation’or‘full evaluation’ Then these options (requirements) are similar to each other.
%--------------------------------------------------------
\bigstrut\\
\cline{2-5} 
& Conflict
& Conflicts~\cite{k_process_centered_1996}, Conflicts\_with~\cite{dahlstedt_requirements_2005}
& Implementation of one requirement negatively impacts another requirement.  
& Increasing security might negatively impact system performance.
%--------------------------------------------------------
\bigstrut\\
\cline{2-5} 
& Be\_exception\_of
& New dependency type
& One requirement describes an exceptional event of another requirement.
&‘‘A user inputs a null username and system reminds him to input his correct username’’ is an exceptional event of ‘‘a user inputs his username and password and system checks validity of his information’’.
%--------------------------------------------------------
\bigstrut\\
\cline{2-5} 
&Evolve\_into
& Replaces~\cite{k_process_centered_1996}, Satisfies~\cite{k_process_centered_1996}, Based\_on~\cite{k_process_centered_1996}, Changes\_to~\cite{dahlstedt_requirements_2005}
&If requirement B is a new version of requirement A, then A evolves into B. This type of dependency is used
to trace and compare different versions of requirement documents.
&‘‘Clients use a desktop PC to upload reports’’ evolves into ‘‘clients use PDA to upload reports’’.
%--------------------------------------------------------
\bigstrut\\
\cline{2-5} 
& Refine
& Refines~\cite{k_process_centered_1996}, Refines\_to~\cite{dahlstedt_requirements_2005}
& One requirement is refined by more specific requirements. 
&‘A valuer submit a valuation report’ is reﬁned as ‘a valuer submits a report through web system’,‘a valuer submits a report through PDA’.
%--------------------------------------------------------
\bigstrut\\
\hline
Additional
&Increase/Decrease\_cost\_of 
& Increase/Decrease\_cost\_of~\cite{dahlstedt_requirements_2005} 
&The implementation of one requirement causes the increase/decrease of the implementation cost of another requirement.
&If one requirement states that ‘no response time should be longer than 5 seconds, it is most likely to increase the cost of  implementing many other requirements.
%--------------------------------------------------------
\bigstrut\\
\cline{2-5} 
&Increase/Decrease\_value\_of 
& Increase/Decrease\_value\_of~\cite{dahlstedt_requirements_2005} 
& The implementation of one requirement causes the increase/decrease of the value to the customer of another requirement. Note that ‘value’ here mainly reﬂects customer’s satisfaction. 
& Users can listen to MP3 when they are browsing photos in a mobile phone. In this case, ‘users can listen to mp3’ increases
customer’s satisfaction of ‘users can browse photos’. 
\bigstrut\\
\Xhline{4\arrayrulewidth}
%--------------------------------------------------------
\end{tabular}}


==> table_types_zhang_2.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet3'
\large\resizebox {1\textwidth }{!}{\begin{tabular}{|r|r|r|r|}
\hline
Category &
  Types in Zhang's model &
  Corresponding types  in  other models &
  Example
  \bigstrut\\
\hline
\multicolumn{1}{|c|}{} &
  \multirow{3}[2]{*}{Constrain} &
  \multirow{3}[2]{*}{Constrain ~\cite{k_process_centered_1996}} &
  \multicolumn{1}{l|}{·     r_1: system should respond to users in 3 seconds}
  \bigstrut[t]\\
 &
   &
   &
  \multicolumn{1}{l|}{·      r_2: users search books using book title or ID}
  \\
 &
   &
   &
  \multicolumn{1}{l|}{·     r_1 constrains r_2}
  \bigstrut[b]\\
\cline{2-4} &
  \multirow{3}[2]{*}{Precede} &
  \multirow{3}[2]{*}{Precondition ~\cite{k_process_centered_1996}, Requires  ~\cite{dahlstedt_requirements_2005}} &
  \multicolumn{1}{l|}{·     r_1: a client initiates a valuation request and the system checks the quality of the request}
  \bigstrut[t]\\
Intrinsic &
   &
   &
  \multicolumn{1}{l|}{·     r_2: users search books using book title or ID}
  \\
 &
   &
   &
  \multicolumn{1}{l|}{·     r_1 precedes r_2}
  \bigstrut[b]\\
\cline{2-4} &
  \multirow{3}[2]{*}{Be similar  to} &
  \multirow{3}[2]{*}{Similar  ~\cite{k_process_centered_1996}, Similar\_to~\cite{dahlstedt_requirements_2005}} &
  \multicolumn{1}{l|}{·     r_1: a system administrator adds a new book record}
  \bigstrut[t]\\
 &
   &
   &
  \multicolumn{1}{l|}{·     r_2: system administrator modifies an old book record. }
  \\
 &
   &
   &
  \multicolumn{1}{l|}{·     r_1 is similar to  r_2 (Book  record  in these  two requirements  is identical).}
  \bigstrut[b]\\
\cline{2-4} &
  \multirow{3}[2]{*}{Conflict} &
  \multirow{3}[2]{*}{Conflicts  ~\cite{k_process_centered_1996}, Conflicts\_with  ~\cite{dahlstedt_requirements_2005}} &
  \multicolumn{1}{l|}{·     r_1: increasing  security}
  \bigstrut[t]\\
 &
   &
   &
  \multicolumn{1}{l|}{·     r_2: improving performance}
  \\
 &
   &
   &
  \multicolumn{1}{l|}{·     r_1 conflicts with  r_2}
  \bigstrut[b]\\
\cline{2-4} &
  \multirow{3}[2]{*}{Be exception of} &
  \multirow{3}[2]{*}{Only in zhang's model} &
  \multicolumn{1}{l|}{·     r_1: A user inputs a null username and  system  reminds  him to input his correct  username }
  \bigstrut[t]\\
 &
   &
   &
  \multicolumn{1}{l|}{·     r_2: a  user  inputs his  username and  password  and  system checks validity of his information}
  \\
 &
   &
   &
  \multicolumn{1}{l|}{·     r_1 is an exception of   r_2}
  \bigstrut[b]\\
\cline{2-4} &
  \multirow{3}[2]{*}{Evolve  into} &
  \multirow{3}[2]{*}{Replaces  ~\cite{k_process_centered_1996}, Satisfies  ~\cite{k_process_centered_1996}, Based  on ~\cite{k_process_centered_1996}, Changes} &
  \multicolumn{1}{l|}{·     r_1:  clients  use a desktop  PC  to upload  reports }
  \bigstrut[t]\\
 &
   &
   &
  \multicolumn{1}{l|}{·     r_2:   clients use PDA to upload reports.}
  \\
 &
   &
   &
  \multicolumn{1}{l|}{·     r_1    evolves into r_2}
  \bigstrut[b]\\
\cline{2-4} &
  \multirow{4}[2]{*}{Refine} &
  \multirow{4}[2]{*}{Refines ~\cite{k_process_centered_1996}, Refines\_to ~\cite{dahlstedt_requirements_2005}} &
  \multicolumn{1}{l|}{·     r_1:  a valuer  submit a valuation report}
  \bigstrut[t]\\
 &
   &
   &
  \multicolumn{1}{l|}{·     r_2:  a valuer  submits a report through web system}
  \\
 &
   &
   &
  \multicolumn{1}{l|}{·     r_3:  a valuer  submits a report through PDA}
  \\
 &
   &
   &
  \multicolumn{1}{l|}{·     r_1 is refined as r_2 and r_3}
  \bigstrut[b]\\
\hline
 &
  \multirow{3}[2]{*}{Increase/Decrease cost of} &
  \multirow{3}[2]{*}{Increase/Decrease\_Cost\-Of~\cite{dahlstedt_requirements_2005}} &
  \multicolumn{1}{l|}{·     r_1:  no response  time  should be longer than  5 seconds}
  \bigstrut[t]\\
 &
   &
   &
  \multicolumn{1}{l|}{·     r_1 is most likely to increase  the cost of implementing many  other  requirements. }
  \\
 &
   &
   &
  
  \bigstrut[b]\\
\cline{2-4}Additional &
  \multirow{3}[2]{*}{Increase/Decrease value  of} &
  \multirow{3}[2]{*}{Increase/Decrease\_Value_\Of ~\cite{dahlstedt_requirements_2005}} &
  \multicolumn{1}{l|}{·     r_1:  users  can  listen  to  music  in a mobile  phone}
  \bigstrut[t]\\
 &
   &
   &
  \multicolumn{1}{l|}{·     r_2:   users can  browse  photos in a mobile phone}
  \\
 &
   &
   &
  \multicolumn{1}{l|}{·     r_1    increases customer satisfaction (value) of  r_2}
  \bigstrut[b]\\
\hline
\end{tabular}}%


==> table_types_zhang_3.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet2'
%\Huge
%\huge
%\LARGE
%\Large
%\large
%\normalsize (default)
%\small
%\footnotesize
%\scriptsize
%\tiny
\LARGE
\rowcolors{1}{}{gray}
\resizebox {1.15\textwidth }{!}{\begin{tabular}{|!{\centering}m{4cm}|!{\centering}m{12.8cm}|!{\centering}m{22cm}|!{\centering}m{25cm}|}
		\Xhline{4\arrayrulewidth}
		\textbf{Category} &
		\textbf{Type} &
		\textbf{Description} &
		\textbf{Example}
		%--------------------------------------------------------
		\bigstrut\\
		\Xhline{4\arrayrulewidth}
		intrinsic
		&  Constrain~\cite{zhang_investigating_2014,k_process_centered_1996}  
		& One requirement is a constraint of another requirement. This kind of dependency can represent crosscutting relationships among requirements.
		& \begin{itemize}
			\item $r_1:$ system should respond to users in 3 seconds
			\item $r_2:$ users search books using book title or ID
			\item $r_1$ constrains $r_2$
		\end{itemize}
		%--------------------------------------------------------
		\bigstrut\\
		\cline{2-4} 
		& Precede~\cite{zhang_investigating_2014}, Precondition~\cite{k_process_centered_1996}, Requires~\cite{dahlstedt2005requirements}
		& If function A precedes function B, A is a precondition of B.
		& \begin{itemize}
			\item $r_1:$ a client initiates a valuation request and the system checks the quality of the request
			\item $r_2:$ users search books using book title or ID
			\item $r_1$ precedes $r_2$
		\end{itemize}
		%--------------------------------------------------------
		\bigstrut\\
		\cline{2-4} 
		& Be\_similar\_to~\cite{zhang_investigating_2014}, Similar~\cite{k_process_centered_1996}, Similar\_to~\cite{dahlstedt2005requirements}
		&\begin{itemize}
			\item a) If two requirements share similar data information, they are similar to each other. 
			\item b) If two requirements complete similar tasks, they are similar to each other.
		\end{itemize}
		&\begin{itemize}
			\item a) System administrator adds a new book re-cord is similar to system administrator modifies an old book record. Book record in these two requirements is identical. 
			\item b) After a client proposes a property valuation request, one valuer can choose from several options to evaluate the property,such as desktop valuation, curbside valuation or full evaluation Then these options (requirements) are similar to each other.
		\end{itemize}
		%--------------------------------------------------------
		\bigstrut\\
		\cline{2-4} 
		& Conflicts~\cite{zhang_investigating_2014,k_process_centered_1996}, Conflicts\_with~\cite{dahlstedt2005requirements}
		& Implementation of one requirement negatively impacts another requirement.  
		& \begin{itemize}
			\item Increasing security might negatively impact system performance.
		\end{itemize}
		%--------------------------------------------------------
		\bigstrut\\
		\cline{2-4} 
		& Be\_exception\_of~\cite{zhang_investigating_2014}
		& One requirement describes an exceptional event of another requirement.
		&\begin{itemize}
			\item $r_1:$ A user inputs a null username and  system  reminds  him to input his correct  username.
			\item $r_2:$ a  user inputs his  username and  password  and  system checks validity of his information.
			\item $r_1$ is an exception of $r_2$. 
		\end{itemize}
		%--------------------------------------------------------
		\bigstrut\\
		\cline{2-4} 
		& Evolve\_into~\cite{zhang_investigating_2014}, Replaces~\cite{k_process_centered_1996}, Satisfies~\cite{k_process_centered_1996}, Based\_on~\cite{k_process_centered_1996}, Changes\_to~\cite{dahlstedt2005requirements}
		&If requirement B is a new version of requirement A, then A evolves into B. This type of dependency is used
		to trace and compare different versions of requirement documents.
		&\begin{itemize}
			\item $r_1:$ clients  use a desktop  PC  to upload  reports.
			\item $r_2:$ clients use PDA to upload reports.
			\item $r_1$ evolves into $r_2$. 
		\end{itemize}
		%--------------------------------------------------------
		\bigstrut\\
		\cline{2-4} 
		& Refines~\cite{zhang_investigating_2014,k_process_centered_1996}, Refines\_to~\cite{dahlstedt2005requirements}
		& One requirement is refined by more specific requirements. 
		&\begin{itemize}
			\item $r_1:$ a valuer submit a valuation report.
			\item $r_2:$ a valuer submits a report through web system.
			\item $r_1$ is refined as $r_2$. 
		\end{itemize}
		%--------------------------------------------------------
		\bigstrut\\
		\hline
		Additional Cost/Value
		& Increase/Decrease\_cost\_of~\cite{zhang_investigating_2014,dahlstedt2005requirements} 
		&The implementation of one requirement causes the increase/decrease of the implementation cost of another requirement.
		&\begin{itemize}
			\item If one requirement states that no response time should be longer than 5 seconds, it is most likely to increase the cost of  implementing many other requirements.
		\end{itemize}
		%--------------------------------------------------------
		\bigstrut\\
		\cline{2-4} 
		& Increase/Decrease\_value\_of~\cite{zhang_investigating_2014,dahlstedt2005requirements} 
		& The implementation of one requirement causes the increase/decrease of the value to the customer of another requirement. Note that value here mainly reflects customers satisfaction. 
		& \begin{itemize}
			\item $r_1:$ users  can  listen  to  music  in a mobile  phone.
			\item $r_2:$ users can  browse  photos in a mobile phone.
			\item $r_1$ increases customer satisfaction (value) of $r_2$. 
		\end{itemize}
		\bigstrut\\
		\Xhline{4\arrayrulewidth}
		%--------------------------------------------------------
	\end{tabular}}
